A Unifying Hierarchy of Valuations with Complements and Substitutes

We introduce a new hierarchy over monotone set functions, that we refer to as $\mathcal{MPH}$ (Maximum over Positive Hypergraphs). Levels of the hierarchy correspond to the degree of complementarity in a given function. The highest level of the hierarchy, $\mathcal{MPH}$-$m$ (where $m$ is the total number of items) captures all monotone functions. The lowest level, $\mathcal{MPH}$-$1$, captures all monotone submodular functions, and more generally, the class of functions known as $\mathcal{XOS}$. Every monotone function that has a positive hypergraph representation of rank $k$ (in the sense defined by Abraham, Babaioff, Dughmi and Roughgarden [EC 2012]) is in $\mathcal{MPH}$-$k$. Every monotone function that has supermodular degree $k$ (in the sense defined by Feige and Izsak [ITCS 2013]) is in $\mathcal{MPH}$-$(k+1)$. In both cases, the converse direction does not hold, even in an approximate sense. We present additional results that demonstrate the expressiveness power of $\mathcal{MPH}$-$k$. One can obtain good approximation ratios for some natural optimization problems, provided that functions are required to lie in low levels of the $\mathcal{MPH}$ hierarchy. We present two such applications. One shows that the maximum welfare problem can be approximated within a ratio of $k+1$ if all players hold valuation functions in $\mathcal{MPH}$-$k$. The other is an upper bound of $2k$ on the price of anarchy of simultaneous first price auctions. Being in $\mathcal{MPH}$-$k$ can be shown to involve two requirements -- one is monotonicity and the other is a certain requirement that we refer to as $\mathcal{PLE}$ (Positive Lower Envelope). Removing the monotonicity requirement, one obtains the $\mathcal{PLE}$ hierarchy over all non-negative set functions (whether monotone or not), which can be fertile ground for further research.

==> algorithmic.tex <==
\ricomment{nice, but in my opinion, better for the introduction. Note that we have to remind ABDR's work here to be fair to the reader. We can also consider putting it as part of the specific introduction for WM, in the section suggested by Vasilis. Currently omitted.}
\Omit{
In this section we demonstrate the usefulness of our hierarchy for algorithmically solving the welfare maximization problem.  While constant factor approximations exist for welfare maximization in the absence of complementarities (see, e.g.,~\cite{LLN, DNS, Feige_Subadditive}), it is not hard to see that complementarities can make the welfare problem as hard as independent set and hence inapproximable to within a linear factor.  Our hierarchy offers a graceful degradation of the approximation guarantee as a function of the degree of complementarity.
}

In this section we present a $1/(k+1)$-approximation algorithm for the welfare maximization problem with $\MOPH$-$k$ valuation functions. Since any instance of the welfare maximization problem is in $\MOPH$-$k$ for some $k \in \mathbb{N}$, our algorithm is actually for any instance of the problem, but with approximation guarantee according its ``$\MOPH$ complexity'' (i.e. its position in the $\MOPH$ hierarchy).
Our algorithm is an LP rounding algorithm.
The rounding uses an idea of \cite{Feige_Subadditive}
combined with a new simple idea of iterative randomized rounding.
The LP relaxation we use is of Dobzinski, Nisan and Schapira \cite{DNS} 
and it uses a demand query oracle\footnote{We recall the definitions of value and demand queries in Appendix~\ref{app:queries}.}.
Although it is common to require a demand query oracle in order to solve the welfare maximization problem, note that in some cases value query oracle is sufficient for our algorithm (see Appendix~\ref{app:polyRepresentationMPH}).
\Omit{
It should be noted, however, that even simple functions may require an exponential number of hypergraphs in their $\MOPH$ representation (see Appendix~\ref{}. For example, it is easy to show that $f(S) = \min[|S|,n/2]$, which is submodular and hence $\MOPH$-$1$, requires exponentially many hypergraphs for any $\MOPH$-$k$ representation of it (for any $k \in \mathbb{N}$). Proof is deferred to Appendix~\ref{app:polyRepresentationMPH}.
}
The LP we are using is the following.
\begin{LP} [Configuration LP] \label{LP:configuration}
\ \\ \\
\textbf{Maximize} $\sum\limits_{i,S} x_{i,S} \cdot w_i(S)$ 
\ \\ \\Subject to:
\begin{description}
\item[Item Constraints:] $\sum\limits_{i,S \mid j \in S} x_{i,S} \leq 1$ for every item $j \in M$.
\item[Player Constraints:] $\sum\limits_{S} x_{i,S} \leq 1$ for every player $i \in P$.
\item[Non-negativity constraints:] $x_{i,S} \geq 0$.
\end{description}
%where $x_{i,S}$ is an indicator variable indicating whether a player gets an item
%(in the relaxation it is the ``amount'' of an item a player gets).
where $x_{i,S}$ indicates the fraction of subset $S \subseteq M$ allocated to agent $i$. 
\end{LP}

We use a two steps rounding technique for this LP (see \cite{DNS}).
By this technique, we firstly compute a randomized tentative allocation
that has in expectation the value of the optimal fractional solution of the LP,
and then do contention resolution to have a feasible allocation
(but, with a possibly lower value).
%We use this technique. We firstly compute a tentative allocation,
The contention resolution we do is new, and it achieves a non-trivial
approximation guarantee, simultaneously, for each of the positive hypergraph functions composing the given $\MOPH$-$k$ function.
Our algorithm is Algorithm~\ref{a:MPH}.
\floatname{algorithm}{Algorithm}
\begin{algorithm}[h]
\caption{Approximate Welfare Maximization with $\MOPH$-$k$ valuations}
\label{a:MPH}
\textsf{Input:} 
\begin{itemize}
\item An instance of the welfare maximization problem with $\MOPH$-$k$ valuation functions.
\item A demand queries oracle for each valuation function $v_i$ (for any $i \in P$).
\end{itemize}
\textsf{Output:} An approximated solution with guarantee $1/(k+1)$.

\begin{algorithmic}[1]
\STATE {Solve LP~\ref{LP:configuration} using the input demand query oracles and set $x_{i,S}$ to be its solution.
		\Omit{\footnote{i.e. the collection of all $x_{i,S}$ for any pair $i, S$ such that $x_{i,S} > 0$.
		It is well known that if the number of constraints is polynomial, there exists a solution
		with polynomial number of strictly positive variables. Since we have only $|P| + |M|$ constraints
		(non-negativity constraints should not be considered), we may assume we have a polynomial
		sized solution.}}}
\STATE 
{
		\textsf{Tentative allocation:}
		Assume without loss of generality that the solution of the LP satisfies all constraints with equality
		(for justification, see \cite{Feige_Subadditive}).
		Assign to each agent $i$ a tentative set according to the probability distribution induced by the
		variables $x_{i,S}$.
		Note that this tentative allocation has the same expected welfare as the LP.
		However, it may be infeasible as agents' sets might overlap.
}
\STATE 
{
		\textsf{Contention resolution:}
		Generate a uniformly random permutation over the agents ${\cal P} =  (p_1, \ldots p_n)$.
		Iteratively resolve contention by allocating at each iteration $1 \leq t \leq n$ all the not yet allocated items 
		to agent $p_t$.
		That is, preference in contention resolution is decided merely by their order in the permutation ${\cal P}$.
}
\end{algorithmic}
\end{algorithm}

\ricomment{It is not a contribution of our paper to solve this LP using demand oracles, so I personally prefer to save space and not detail it. I also prefer to defer definitions of oracles to appendix, since there is no need to understand them in order to understand our main message of this section. I also stated differently the necessity of demand oracles to stress it is common. About mentioning the spectra example, it may be nice to add it (perhaps to the appendix I created for polynomial representation of $\MOPH$?).}
\Omit{
\paragraph{Solving the LP.} The configuration LP has exponentially many variablies but only polynomially many constraints.  Hence it can be solved through duality given access to {\it demand oracles}: i.e., an oracle that returns, for any ``prices'' $p_j$ for items $j\in M$ and any agent valuation $v_i$, a subset of items $S\subseteq M$ maximizing $v_i(S)-\sum_{j\in S}p_j$.  The existence of efficient demand oracles (both for XoS valuations and general $\MOPH$-$k$ valuations) depends on the representation of the valuation functions.  If the valuation is supported on polynomially many positive hypergraphs, then one can solve the demand query on each hypergraph separately using supermodular function maximization\footnote{Simply subtract the item prices from the corresponding vertices and then observe the resulting graph (which potentially has negative vertex weights) defines a supermodular function.  Supermodular function maximization is equivalent to submodular function minimization, and is well-known to be solvable in strongly polynomial time.} and then return the maximum.  While certain natural valuation classes have polynomial representations (e.g., the natural generalization of the spectra example of Figure~\ref{} to multiple frequencies), others are not (e.g., the $\MOPH$-$1$ valuation function $v(S)=\min\{|S|,n/2\}$ which assigns a value of one to each aquired item up to a cap of $n/2$).  This technique only applies to valuation functions with polynomial representations, or to settings in which the algorithm has access to a demand oracle.
}

\begin{prop} \label{p:algorithmMOH}
Algorithm~\ref{a:MPH} computes a feasible assignment with approximation guarantee of $1/(k+1)$.
\end{prop}

\begin{proofsk}
Firstly, note that the solution is feasible, since any item is allocated at most once.
We upper bound the approximation guarantee.
The sum of values of tentative sets preserve, in expectation, the value of the optimal welfare
returned by \ref{LP:configuration} . 
Consider now an arbitrary player and his tentative set $T$. This set attained its value according to some positive hypergraph $H$ that has no edges of rank larger than $k$. Consider an arbitrary edge of $H$ contained in $T$, and let $r \leq k$ be its rank. We claim that its expected contribution (expectation taken over random choices of other players and random permutation) towards the final welfare is at least $1/(r+1)$ of its value. The expected number of other players who compete on items from this edge is at most $r$ (by summing up the fractional values of sets that contain items from this edge). Given that there are $\ell$ other competing players, the player gets all items from the edge with probability exactly $1/(\ell + 1)$. As the expectation of $\ell$ is at most $r$, the expectation of $1/(\ell+1)$ is at least $1/(r+1)$ (by convexity). The proof follows from linearity of expectation.
\end{proofsk}

\ricomment{I also find it a good idea to state this result as a Theorem, but I personally think we should put it in the introduction/preliminaries (in our results/contribution) and then we can reference it in the beginning of this section.
We can also mention there the result of ABDR with a comparison.}
\Omit{
\begin{theorem}
If all agents have $\MOPH$-$k$ valuations, then there is a polynomial-time algorithm which, given access to demand oracles for the valuations, computes an allocation of items to agents that is a $1/(k+1)$-approximation to the maximum welfare.
\end{theorem}
}

\subsubsection{Lower bounds}
\begin{theorem} \label{t:integralityGap}
Let $k \in \mathbb{N}$ be such than $k-1$ is a power of prime. 
Then, there exists an instance of the welfare maximization problem with positive hypergraph function of rank $k$ and integrality gap $k - 1 + \frac{1}{k}$ for Linear Program~\ref{LP:configuration}.
Note that such an instance is in particular $\MOPH$-$k$.
\end{theorem}
We defer the proof of Theorem~\ref{t:integralityGap} to Appendix~\ref{app:integralityGapWMP}.

\begin{theorem} \label{t:hardness} %TODO: MOH-k vs MOH-r, approximation guarantees/ratio and also 1/d or d.
It is $\NP$-hard to approximate the welfare maximization problem with $\MOPH$-$k$ valuations with approximation guarantee of $\Omega(\frac{\ln k}{k})$.
\end{theorem}

Theorem~\ref{t:hardness} is true even in the single minded case as observed by \cite{Feige2013}.
They use an approximation preserving reduction from $k$-set packing together with hardness results of \cite{HSS}.
Similar in nature results have also been found by Abraham et al. \cite{Abraham2012}, using hardness of independent set in bounded degree graphs.

==> algorithmic_-_Nicole.tex <==

In this section we demonstrate the usefullness of our hierarchy for algorithmically solving welfare maximization problems.  While constant factor approximations exist for welfare maximization in the absence of complementarities (see, e.g., Fiege~\cite{}), it's not hard to see that complementarities can make the welfare problem as hard as independent set and hence inapproximable to within a linear factor.  Our hierarchy offers a graceful degradation of the approximation as a function of the degree of complementarity.  

We follow the approximation technique introduced by Feige~\cite{} for XoS (i.e., $\MOPH$-$1$) valuation functions.  This paper showed that, when all bidders have XoS valuation functions, the maximum welfare can be approximated to within a constant given a certain type of access to the valuations.  At a high level, the technique works as follows: define a {\it configuration linear program} (LP) by introducing a variable $x_{i,S}$ for every agent $i$ and subset of items $S$.  Given the valuation profile $v_i$ of each agent $i$, the configuration LP is:
\begin{eqnarray*}
&\ &\max\sum\limits_{i,S}v_i(S)\cdot x_{i,S}\quad\mathrm{\ subject\ to\ }\\
&\ &\sum\limits_{S} x_{i,S} \leq 1\quad\quad\forall i\in P\\
&\ &\sum\limits_{i,S \mid j \in S} x_{i,S} \leq 1\quad\quad\forall j\in M.
\end{eqnarray*}
where the first constraint guarantees no player is allocated more than one set and the second guarantees no item belongs to more than one set.  This LP provides an upper bound on the optimal welfare.  To find a solution that approximates the optimal welfare, we first must solve this LP and then round it.

\paragraph{Solving the LP.} The configuration LP has exponentially many variablies but only polynomially many constraints.  Hence it can be solved through duality given access to {\it demand oracles}: i.e., an oracle that returns, for any ``prices'' $p_j$ for items $j\in M$ and any agent valuation $v_i$, a subset of items $S\subseteq M$ maximizing $v_i(S)-\sum_{j\in S}p_j$.  The existence of efficient demand oracles (both for XoS valuations and general $\MOPH$-$k$ valuations) depends on the representation of the valuation functions.  If the valuation is supported on polynomially many positive hypergraphs, then one can solve the demand query on each hypergraph separately using supermodular function maximization\footnote{Simply subtract the item prices from the corresponding vertices and then observe the resulting graph (which potentially has negative vertex weights) defines a supermodular function.  Supermodular function maximization is equivalent to submodular function minimization, and is well-known to be solvable in strongly polynomial time.} and then return the maximum.  While certain natural valuation classes have polynomial representations (e.g., the natural generalization of the spectra example of Figure~\ref{} to multiple frequencies), others are not (e.g., the $\MOPH$-$1$ valuation function $v(S)=\min\{|S|,n/2\}$ which assigns a value of one to each aquired item up to a cap of $n/2$).  This technique only applies to valuation functions with polynomial representations, or to settings in which the algorithm has access to a demand oracle.

\paragraph{Rounding the LP.} The rounding proceeds in two steps.  First each agent $i$ is assigned a tentative set $S'_i$ according to the probability distribution induced by the variables $x_{i,S}$.  Note this tentative allocation has the same expected welfare as the LP.  However, it may be infeasible as agents' sets might overlap.  We must resolve these contentions.  To do so, we generate a uniformly random permutation $\pi$ over the agents and then at each step $t$ for $1\leq t\leq n$, assign agent $i=\pi(t)$ items $S_i=S'_i\setminus\{\cup_{i'=\pi(1)}^{\pi(t-1)}S_{i'}\}$, i.e., those items in his tentative set that have not already been allocated.  Feige~\cite{} showed that this contention resolution didn't lose much welfare as \nicomment{some intuition}.  In our setting, we must modify the analysis to account for the complementarities.  The following lemma shows that we lose at most a factor of $k+1$ in this rounding when all agents have $\MOPH$-$k$ valuations:

\begin{lemma}
approximation.
\end{lemma}
\begin{proof} [Sketch]
\nicomment{massage me.}
Firstly, note that the solution is feasible, since any item is allocated at most once.
We upper bound the approximation guarantee.
The sum of values of tentative sets preserve, in expectation, the value of the optimal welfare
returned by \ref{LP:relaxation} . 
Consider now an arbitrary player and his tentative set $T$. This set attained its value according to some positive hypergraph $H$ that has no edges of rank larger than $k$. Consider an arbitrary edge of $H$ contained in $T$, and let $r$ be its rank. We claim that its expected contribution (expectation taken over random choices of other players and random permutation) towards the final welfare is at least $1/(r+1)$ of its value. The expected number of other players who compete on items from this edge is at most $r$ (by summing up the fractional values of sets that contain items from this edge). Given that there are $\ell$ other competing players, the player gets all items from the edge with probability exactly $1/(\ell + 1)$. As the expectation of $\ell$ is at most $r$, the expectation of $1/(\ell+1)$ is at least $1/(r+1)$ (by convexity). The proof follows from linearity of expectation.
\end{proof}


The above discussion yields the following result.
\begin{theorem}
If all agents have $\MOPH$-$k$ valuations, then there is a polynomial-time algorithm which, given access to demand oracles for the valuations, computes an allocation of items to agents that is an $O(k)$ approximation to the maximum welfare.
\end{theorem}

\nicomment{Defer integrality gap and hardness to appendix and reference them here.}
\vscomment{Old stuff are omitted in the tex file.}
\Omit{
\paragraph{Old Stuff.} present a $1/(k+1)$-approximation algorithm for the welfare maximization problem with $\MOPH$-$k$ valuation functions. Since any instance of the welfare maximization problem is in $\MOPH$-$k$ for some $k \in mathbb{N}$, our algorithm is actually for any instance of the problem, but with approximation guarantees according its ``$\MOPH$ complexity''.
Our algorithm is an $LP$ rounding algorithm.
The rounding uses an idea of \cite{Feige_Subadditive}
combined with a new idea of iterative randomized rounding.
The LP relaxation we use is of Dobzinski, Nisan and Schapira \cite{DNS} 
and it uses a demand query oracle.
Although it is common to require a demand queries oracle in order to solve the welfare maximization problem, note that in some cases value queries oracle is sufficient in our case, as we show in the next proposition.

\vsedit{
We recall the definitions of basic types of queries for set functions.
% and introduce dependency and supermodular dependency queries oracle.
Let $f: 2^S \to \nonnegR$ be a set function.
\begin{defn} [Value queries]
{\em Value queries} are the following:
\\\textsf{Input:} A subset $S' \subseteq S$.
\\\textsf{Output:} $f(S')$.
\end{defn}
\begin{defn} [Demand queries]
{\em Demand queries} are the following:
\\\textsf{Input:} A cost function $c: S \to \nonnegR$.
\\\textsf{Output:} A subset $S' \subseteq S$ maximizing $f(S') - \sum_{j \in S'} c(j)$.
\end{defn}
Note that demand queries are strictly stronger than value queries (see~\cite{BlumrosenNisan}).}

\begin{prop}
Given an $\MOPH$-$k$ set function with a representation that has at most polynomially many positive hypergraphs, each with at most polynomially many hyperedges, one can answer demand queries in polynomial time.
%TODO: consider mentioning here we need value queries.
\end{prop}

\begin{proof}
As observed in \cite{Abraham2012}, answering a demand query on one hypergraph is a supermodular maximization task, or equivalently, submodular minimization. Hence by known results, it can done in polynomial time (in fact, value queries suffice for this). 
If there are several hypergraphs, compute an answer for each hypergraph separately, and return the best answer.
\end{proof}

It should be noted, however, that even simple functions may require an exponential number of hypergraphs in their representation.

\begin{prop}
Every MOPH representation (regardless of rank) of the submodular function $f(S) = \min[|S|,n/2]$ (which is in $\MOPH$-$1$) requires exponentially many hypergraphs.
\end{prop}

\begin{proof}
Consider two different sets $S$ and $T$ with $|S| = |T| = n/2$. Let $h$ be an arbitrary supermodular function (hence any positive hypergraph qualifies here) satisfying $h(Q) \le f(Q)$ for every set $Q$. We claim that either $h(S) \not= f(S)$ or $h(T) \not= f(T)$. This proves that at least ${n \choose n/2}$ hypergraphs are needed.

To prove the claim observe that $f(S \cap T) < n/2$ and $f(S \cup T) = n/2$. Suppose for the sake of contradiction that $h(S) = h(T) = n/2$. Then by supermodularity  $h(S \cap T) + h(S \cup T) \ge n$, implying that either $h(S \cap T) > f(S \cap T)$ or $h(S \cup T) > f(S \cup T)$, a contradiction.
\end{proof}
%It is well known that the maximum welfare configuration LP can be solved in polynomial time if one is equipped with %demand queries. 
%The reason is that demand queries can serve as separation oracles in the dual program.
%We therefore obtain the following corollary.
 
%\begin{corollary}
%For polynomial MOPH valuation functions, the maximum welfare configuration LP can be solved in polynomial time.
%\end{corollary}

%We now show that for polynomial MOPH-k valuation functions, one can obtain a fraction of at least $1/(k+1)$ of the %optimal welfare in polynomial time.
\ricomment{I suggest adding a (sub)section with our results and state their the Theorem, perhaps with comparisons to e.g. ABDR's paper.}
%\begin{theorem}
%For MOPH-k valuation functions, the maximum welfare configuration LP can be rounded preserving a fraction of at least %$1/(k+1)$ of the welfare.
%\end{theorem}

The LP we use is the following.
\begin{LP} [Configuration LP] \label{LP:relaxation}
\ \\ \\
\textbf{Maximize} $\sum\limits_{i,S} x_{i,S} \cdot w_i(S)$ 
\ \\ \\Subject to:
\begin{description}
\item[Item Constraints:] $\sum\limits_{i,S \mid j \in S} x_{i,S} \leq 1$ for every item $j \in M$.
\item[Player Constraints:] $\sum\limits_{S} x_{i,S} \leq 1$ for every player $i \in P$.
\item[Non-negativity constraints:] $x_{i,S} \geq 0$.
\end{description}
where $x_{i,S}$ is an indicator variable indicating whether a player gets an item
(in the relaxation it is the ``amount'' of an item a player gets).
\end{LP}

We use a two steps rounding technique for this LP (see \cite{DNS}).
This technique firstly computes a randomized tentative allocation
that has in expectation the value of the optimal fractional solution of the LP,
and then does contention resolution to have a feasible solution
(but with a lower value).
We use this technique. We firstly compute a tentative allocation,
and then use a new idea of contention resolution that achieves a non-trivial
approximation guarantee, simultaneously, for each of the positive hypergraph functions composing the given $\MOPH$-$k$ function.

Our algorithm is the following:
\floatname{algorithm}{Algorithm}
\begin{algorithm}[H]
\caption{Approximate Welfare Maximization with $\MOPH$-$k$ valuations}
\label{a:MOH}
\textsf{Input:} 
\begin{itemize}
\item An instance $\II(P, M, v)$ of the welfare maximization problem with $\MOPH$-$k$ valuation functions.
\item A positive integer $r$.
\item A demand queries oracle for each valuation function $v_p$ (for any $p \in P$).
\end{itemize}
\textsf{Output:} An approximated solution with guarantee $1/(k+1)$.

\begin{algorithmic}[1]
\STATE {Solve LP~\ref{LP:relaxation} using the input demand queries oracles and set $x_{i,S}$ to be its solution.
		\footnote{i.e. the collection of all $x_{i,S}$ for any pair $i, S$ such that $x_{i,S} > 0$.
		It is well known that if the number of constraints is polynomial, there exists a solution
		with polynomial number of strictly positive variables. Since we have only $|P| + |M|$ constraints
		(non-negativity constraints should not be considered), we may assume we have a polynomial
		sized solution.}}
\STATE 
{
		\textsf{Tentative allocation:}
		Assume without loss of generality that the solution of the LP satisfies all constraints with equality
		(for justification, see \cite{Feige_Subadditive})
		Set $TentativeAllocation$ to be an allocation giving to any player $p \in P$
		a subset $S \subseteq M$, where subset $S$ is chosen for player $p$ with probability $x_{p, S}$.
}
\STATE 
{
		\textsf{Contention resolution:}
		Generate a uniformly random permutation over the players $\PP =  (p_1, \ldots p_n)$.
		Iteratively resolve contention by allocating at each iteration $1 \leq i \leq n$ all the not yet allocated items to player $p_i$.
		That is, preference in contention resolution is decided merely by their order in $\PP$.
}
\end{algorithmic}
\end{algorithm}

\begin{prop} \label{p:algorithmMOH}
Algorithm~\ref{a:MOH} computes a legal assignment with approximation guarantee of $k+1$.
\end{prop}
\begin{proof} [Sketch]
Firstly, note that the solution is feasible, since any item is allocated at most once.
We upper bound the approximation guarantee.
The sum of values of tentative sets preserve, in expectation, the value of the optimal welfare
returned by \ref{LP:relaxation} . 
Consider now an arbitrary player and his tentative set $T$. This set attained its value according to some positive hypergraph $H$ that has no edges of rank larger than $k$. Consider an arbitrary edge of $H$ contained in $T$, and let $r$ be its rank. We claim that its expected contribution (expectation taken over random choices of other players and random permutation) towards the final welfare is at least $1/(r+1)$ of its value. The expected number of other players who compete on items from this edge is at most $r$ (by summing up the fractional values of sets that contain items from this edge). Given that there are $\ell$ other competing players, the player gets all items from the edge with probability exactly $1/(\ell + 1)$. As the expectation of $\ell$ is at most $r$, the expectation of $1/(\ell+1)$ is at least $1/(r+1)$ (by convexity). The proof follows from linearity of expectation.
\end{proof}

\subsection{Lower bounding the integrality gap}
\begin{theorem} \label{t:integralityGap}
Let $k \in \mathbb{N}$ be such than $k-1$ is a power of prime. 
There exists an instance of the welfare maximization problem with positive hypergraph function of rank $k$ and integrality gap $k - 1 + \frac{1}{k}$ for Linear Program~\ref{LP:relaxation}.
Note that such an instance is in particular $MOPH$-$k$.
\end{theorem}

\begin{proof} %TODO: verify
We take the as the hypergraph representation of all player the players to be based on the finite projective plane of order $k-1$ (which exists since $k-1$ is a power of a prime).
Instead of points we have vertices and instead of lines we have hyperedges of rank $k$.
We have $(k-1)^2+(k-1)+1 = (k-1)^2 + k$ vertices (items).
We have also $(k-1)^2+k$ hyperedges.
Any~2 hyperedges have a vertex in common.
Any non-zero hyperedge contains exactly $k$ vertices.
Any vertex is contained in exactly $k$ hyperedges.
Our instance contains $(k-1)^2+k$ players where each player has value~1 to one of the hyperedges of rank $k$ and~0 to the rest (distinct hyperedges for distinct players).
Note that there are no non-zero hyperedges of any other rank.
An optimal integral solution is an allocation of one of the hyperedges to the player who has value~1 for it.
This solution has value~1.
However, there exists a better fractional solution.
Any player gets a fraction of $\frac{1}{k}$ of all the vertices (items) in the hyperedge of value~1 by her valuation.
It is easy to verify this is a feasible fractional solution.
Its value is $\frac{(k-1)^2+k}{k} = k - 1 + \frac{1}{k}$ as desired.
This concludes the proof of Theorem~\ref{t:integralityGap}.
\end{proof}

\subsection{Hardness}
\begin{theorem} \label{t:hardness} %TODO: MOH-k vs MOH-r, approximation guarantees/ratio and also 1/d or d.
It is $NP$-hard to approximate the welfare maximization problem with $\MOPH$-$k$ valuations with approximation guarantee of $\Omega(\frac{\ln k}{k})$.
\end{theorem}
Theorem~\ref{t:hardness} is true even in the single minded case as observed by \cite{FeigeIzsak}.
They use an approximation preserving reduction from $k$-set packing together with hardness results of \cite{HazanSafraSchwartz}.
Similar in nature results have also been found by Abraham et al. \cite{ABDR}, using hardness of independent set in bounded degree graphs.
}

==> definitions-hypergraph.tex <==


To this end, we introduce a new hierarchy of valuation classes that includes all monotone set functions.
We refer to the $k^{\text{th}}$ class in this hierarchy as {\em Maximum over Positive Hypergraphs} of degree $k$ ($\MOPH$-$k$), where $k \geq 1$ is a parameter reflecting the degree of complementarity.
This class is syntactic: a set function is $\MOPH$-$k$ if it can be expressed as a maximum over an arbitrary set of $\PH$-$k$ functions, introduced by Abraham, Babaioff, Dughmi and Roughgarden \cite{Abraham}.

A hypergraph representation $h$ of a set function $f$ is a set function that satisfies $f(S) = \sum_{T \subseteq S} h(T)$. 
It is easy to verify that any set function $f$ admits a unique hypergraph representation and vice versa.
A set $S$ such that $h(S) \neq 0$ is said to be a {\em hyperedge} of $h$.
If $h(S) \geq 0$ for any $S \subseteq M$, then we refer to such a function as a \emph{positive hypergraph function}.
\ricomment{Uncommented the next sentence. Seems important to me (we call it *hypergraph* representation, and I also think we use it.}
Pictorially, the hypergraph representation can be thought of as a weighted hypergraph, with weights on hyperedges, such that the value of a certain set $S$ is the the total value of all hyperedges contained in $S$. 
The {\em rank} of a hypergraph representation is the cardinality of its largest hyperedge.
Similarly, the {\em positive rank} (respectively, {\em negative rank}) of $h$ is the cardinality of its largest positive (respectively, negative) hyperedge.
We also use ``rank'' and ``positive/negative rank'' for set functions, meaning the respective rank of their (unique) hypergraph representation.
\ricomment{Do we use Hypergraph-$r$}
A hypergraph function with rank at most $r$ belongs to Hypergraph-$r$. 
A positive hypergraph function with rank at most $r$ belongs to (Positive Hypergraph-r) ($PH$-$r$).



==> demandqueries.tex <==
\subsection{$\MOPH$ as a useful representation}

An explicit description (as a truth table) of a set function over $m$ items contains $2^m - 1$ entries. However, one is typically more interested in those set functions that have implicit descriptions of size polynomial in $m$ (which by a simple counting argument constitute only a small fraction of all possible set functions). A set function may have several different polynomial size descriptions, that differ wildly in their usefulness. For example, a useful description of a linear function simply lists the values of all items, whereas a rather useless description is to list $m$ NP-hard optimization problems, with the intended interpretation that the value of the $i$th item is equal to the value of the optimal solution of the $i$th problem.

Given a description of a set function $f$, a ``minimal" notion of usefulness is that of having the ability to answer {\em value queries}, namely, to have a fast (polynomial time) algorithm that given a set $S$ as input, returns $f(S)$. Such an algorithm is referred to as a {\em value oracle} for $f$. Ideally, the value oracle has a polynomial size implementation, say, as a circuit of size polynomial in $m$. However, in the context of combinatorial auctions, one may also imagine using exponential size implementations of value oracles: an agent may hold a representation of his own valuation function $f$ as a truth table. This representation may be too long to be communicated in its entirety to the welfare maximization algorithm, but the agent may answer value queries quickly upon request, by having random access (rather than sequential access) to this table.

Another notion of usefulness that comes up naturally in the context of combinatorial auctions is that of having the ability to answer {\em demand queries}, namely, to have a fast (polynomial time) algorithm that given a list of item prices $p_i$ as input, returns the set $S$ that maximizes $f(S) - \sum_{i\in S} p_i$. Such an algorithm is referred to as a {\em demand oracle} for $f$. A demand oracle is at least as difficult to implement as a value oracle, because value queries can be implemented using demand queries (to query for the value of $f(S)$, use a demand query in which items in $S$ are priced at~0 and all other items have prohibitively large prices).

It is shown in~\cite{FeigeJozeph2014}
that even some submodular functions that have a polynomial representation do not have any polynomial size implementation of demand oracles (not even oracles that answer demand queries approximately), unless NP has polynomial size circuits. In fact, there are such functions that do not have any polynomial size implementation of value oracles (unless NP has polynomial size circuits). Hence not all functions in $\MOPH$-1 have useful representations, not even those functions that have a polynomial representation.

%In the context of $\MOPH$ it is especially interesting to consider those function that have a polynomial size $\MOPH$ representation (rather than an arbitrary polynomial size representation).
A function $f$ is said to have a polynomial size $\MOPH$ representation is it can be represented as a maximum over polynomially many positive hypergraphs, where each hypergraph is of polynomial size. Interestingly, a polynomial size $\MOPH$ representation is always a useful representation.

\begin{proposition}
Given a polynomial size $\MOPH$ representation of a set function $f$, one can answer demand queries in polynomial time.
\end{proposition}

[Move proof from Section 5.1 here]



==> expressiveness.tex <==
% !TEX root=complements.tex

\Omit{Crucially, since both the algorithmic and game theoretic applications of our hierarchy will produce positive results that depend on the allowable level of the hierarchy, low levels of complementarity are highly desirable.

Our hierarchy is by no means the first hierarchy that addresses the degree of complementarity of a set function. Three notable other measures have been used in the literature: the supermodular degree of Feige and Izsak \cite{Feige2013}, the size of the single-minded functions used as basic building blocks of XOR and OR functional operations \cite{Sandholm2002} and the rank of the hypergraph representation of the function \cite{Acemoglu2012}. All these measures imply an hierarchy of monotone set functions.

We show that our hierarchy is strictly more expressive than the first two hierarchies, with the ``gap" of expressiveness growing as the number of items. The comparison to the third measure is more subtle and significantly more challenging. We show that under some natural assumptions on the structure of the hypergraph representation our measure of complementarity is close to the rank of the hypergraph representation. Interestingly, our results imply that in many cases only the positive rank of the hypergraph representation matters, while the negative rank can be arbitrary. Moreover, we give examples where the rank in the hypergraph representation can be significantly higher than the corresponding rank in our measure. We leave the general comparison between these hierarchies as an open problem.
}

In this Section we study the expressive power of the $\MOPH$ hierarchy, with an eye toward proving the statements in Theorem~\ref{thm:expressiveness}.  We will describe how $\MOPH$ compares to other classes of functions from the literature that have been used to describe complementarity.  We will also describe our partial progress toward resolving Conjecture~\ref{conj:quadratic}.

%Our hierarchy is not the first to address the degree of complementarity of a set function.
%However, as asserted by Proposition~\ref{prop:incompatible}, previous hierarchies are mutually incompatible in the sense that functions in very low levels of one hierarchy cannot be approximated well even at relatively high levels of other hierarchies.
%This is discussed further in Appendix~\ref{sec:incompatible}.
%In this section we show that the $\MOPH$ hierarchy is strictly more expressive than previous hierarchies.
%Essentially, we establish the statements that compose Theorem~\ref{thm:expressiveness}.

We begin by describing the positive lower envelope technique, which is the primary technical tool used throughout the section.  We then relate $\MOPH$ to supermodular degree and to special cases of hypergraph valuations.

\paragraph{Positive Lower Envelope Technique.}
\Omit{In most of the results in this section we will be showing that a class of set functions always admits an $\MOPH$-$k$ representation for some $k$.}
Proving that a particular set function $f:2^M\to \nonnegR$ can be expressed as $\MOPH$-$k$ requires constructing a set of $\PH$-$k$ valuations that constitutes the index set $\Ell$ over which the maximum is taken.
In what follows we present a canonical way of constructing the set $\Ell$.
The idea is to create a $\PH$-$k$ function for every subset $S$ of the ground set $M$.
The collection of these $\PH$-$k$ functions, one for each subset, constitutes a valid $\MOPH$-$k$ representation if they adhere to what we define as Positive Lower Envelopes.
%\footnote{The existence of such Positive Lower Envelopes, actually gives rise to a hierarchy of set functions
%that goes beyond monotone functions, and coincides with $\MOPH-k$ for monotone ones.
%For conciseness, we defer this discussion to Section~\ref{sec:non-monotone}.}.

\begin{defn} [Positive Lower Envelope (PLE)] \label{def:PLE}
Let $f: 2^M \to \nonnegR$ be a monotone set function.
A positive lower envelope (PLE) of $f$ is any positive hypergraph function $g$ such that:
\begin{itemize}
\item $g(M) = f(M)$.
\item For any $S \subseteq M$, $g(S) \leq f(S)$. [No overestimate]
\end{itemize}
\end{defn}

%\ricomment{omitted. The text above seems to me much better and also sufficient together with some additions I made.}
\Omit{
In order to prove that a function is in $\MOPH$-$k$, for every set $S \subseteq M$, we consider the function restricted to that subset $S$ and construct a lower envelope for this restriction.  We then take the maximum over these lower envelopes. The first property will ensure that no set is being overestimated.
The second property will ensure the existence of at least one function for which the desired value is obtained; thus no underestimation occurs either. The following characterization is almost self evident; its formal proof is deferred to Appendix~\ref{app:ple-technique}.
}

Before presenting the characterization, we need the following definition.
A function $f:2^M \to \nonnegR$ {\em restricted to a subset $S$}, $S \subseteq M$, is a function $f_S: 2^S \subseteq \nonnegR$ with $f_S(S') = f(S')$ for every $S' \subseteq S$.
We show that a monotone set function is in $\MOPH$-$k$ if and only if $f_S$ admits a $PLE$ of rank $k$ for every set $S \subseteq M$.
This characterization follows directly from the following two propositions, whose proofs are deferred to Appendix~\ref{app:ple-technique}.

\begin{prop} \label{p:PLEtoMOH} \label{lem:lower-envelope}
Every monotone set function $f$ such that $f_S$ admits a lower envelope of rank $k$ for every set $S \subseteq M$ is in $\MOPH$-$k$.
\end{prop}

%Note that the other direction is also true.
\begin{prop} \label{p:MOHtoPLE}
Every function $f$ that is in $\MOPH$-$k$ is monotone.
Moreover, For every set $S \subseteq M$, $f_S$ admits a positive lower envelope of rank $k$.
\end{prop}

%That is, any monotone set function is in $\MOPH$-$k$ if and only if it admits a positive lower envelope of rank $k$ for %any restriction of it to a subset of its groundset.

%\mfcomment{I moved the proof and discussion to an appendix.
%This section in the appendix should be edited a little to prove the characterization.
%Currently it proves only one side.}


\subsection{Supermodular Degree Hierarchy}
\label{sec:supermodular}
\input{supermodular}

%\mfcomment{I commented out the section on XOS-k for now.}
\Omit
{\subsection{XORs and ORs of Single-Minded Valuations}
\input{xos-k}
}

\subsection{Hypergraph Functions with Positive and Negative Hyperedges}
\label{sec:positive-and-negative}
\input{positive-and-negative}

\subsection{Limitations of the $\MOPH$ hierarchy}
\label{sec:limitations}
\input{limitations}

%\blcomment{I recommend that we cut the rest of the section.  The last result, below, doesn't seem as important as the rest.  Do we use it?  If we do keep it, we should comment on why it is interesting.}
%
%\bledit{Finally, for the special case of graphical valuations with positive and negative edge weights \cite{Acemoglu2012}, we can prove a stronger version of Theorem \ref{thm:hypergraph-vs-MOPH}: such a valuation can be expressed as a monotone submodular function plus a graphical valuation with positive weights.}
%
%\begin{theorem}\label{thm:graphical-decomp}
%Any monotone graphical valuation with positive and negative edges can be decomposed as the sum of a monotone submodular function
%and a graphical valuation with only positive weights.
%\end{theorem}
%\begin{proof}
%Let $v(\cdot)$ be a monotone graphical valuation (with positive and negative edges).
%For every $S \subseteq [m]$, let $v_1(S)$ be the valuation induced by the weights of the nodes and the negative edges; i.e., $v_1(S) = \sum_{j\in S}w_j+\sum_{e\in E_S: w_e<0}w_e$, and let $v_2(S)$ the valuation induced by the positive edges; i.e., $v_2(S) = \sum_{e\in E_S:w_e\geq 0}w_e$. Obviously, it holds that $v(S) = v_1(S)+v_2(S)$. Additionally, $v_2(S)$ is, by definition, a graphical valuation with only positive edges. Thus it remains to show that $v_1(S)$ is a monotone submodular valuation.
%
%The submodularity of $v_1(\cdot)$ can be easily verified: for any sets $S,T$ such that $S\subseteq T$ and an item $j\notin S,T$, since the weight of every edge in $v_1(\cdot)$ is negative, it follows that
%\begin{align*}
%v(j~|~S) = w_j + \sum_{k\in S}w_{(j,k)}\geq w_j +\sum_{k\in T}w_{(j,k)}=v(j~|~T).
%\end{align*}
%To show that $v_1(\cdot)$ is monotone, it suffices to show that the marginal contribution of any item $j$ to any given set $S$ is non-negative.
%We will simply show that $v_1(j~|~S)=w_j+\sum_{k\in S}w_{(j,k)} = w_j +\sum_{k\in S:w_{(j,k)}<0}w_{(j,k)}\geq 0$. Let $T=\{k\in S:w_{(j,k)}<0\}$.
%Now observe that when adding $j$ to $T$ the marginal contribution under valuation $v_1(\cdot)$ coincides with the marginal contribution
%with respect to $v(\cdot)$. Thus by monotonicity of $v(\cdot)$ we get: $v_1(j~|~S)=v_1(j~|~T)=v(j~|~T)\geq 0$.
%\end{proof}

%\vscomment{I removed the task valuations. I think it's a very natural class, but is not so well-established and lacks the heaviness of previous comparisons, so most probably not worth it in the main text. Don't know where to mention it.}
%\subsection{Task Valuations}
\Omit{\subsection{Task Valuations}
Last we give another natural class of complementary valuations that can be related to $\MOPH$-$k$ valuations and which we will refer to as $k$-task valuations: there is a set of tasks $\mathcal{T}$ that the player wants to accomplish. Each task $t$ is associated with a collection of sets of items $C_t$, each set of size at most $k$. A player can complete the task $t$ only if he obtains some of the sets in $C_t$ and he gets a value of $w_t(c_t)$ for completing
the task with set $c_t\in C_t$. The value of a player for a set $S$ is the sum of all tasks that he can accomplish with the items in $S$, each task being
accomplished in the best possible way.  To simplify notation we can think that the empty set is always part
of $C_t$, but has an associated value of $0$: $w(\emptyset)=0$. Then a player's value can be written as
%\begin{equation}
$v(S) = \sum_{t\in \T}\max_{c_t\in C_t: c_t\subseteq S}w_t(c_t).$
%\end{equation}
Such a class of valuations captures the class of scheduling valuations studied in \cite{Reeves2005}. In scheduling valuations a player has a task to complete
that requires $k$ time slots from some resource. The value of a player for winning less than $k$ slots is $0$ and his valuations for winning a set of at least $k$ slots is the smallest time by which he can complete his task, i.e. the $k$-th smallest slot that he won.

\begin{theorem}\label{thm:task-valuations}
A $k$-task valuation is $\MOPH$-$k$.
\end{theorem}
\begin{proof}
We will create one valuation for each possible combination of ways of accomplishing each task. Thus each valuation $\ell\in \Ell$ will be associated with a vector $c=(c_1,\ldots,c_{|\mathcal{T}|})$, such that $c_t\in C_t$. We will now create a $k$-hypergraph valuation associated with vector $c$. Each set $c_t$ will be associated with a hyperedge $e_t^c\in E_c$ with weight $w_{e_t^c}^c=w_t(c_t)$. Consider a set of items $S$ and for each $t\in \T$, let $c_t^S=\arg\max_{c_t\in \C_t: c_t\subseteq S}w_t(c_t)$ and let $c^S=(c_t^S)_{t\in \T}$. Thus:
$$v(S) =\sum_{t\in \T}\max_{c_t\in C_t} w_t(c_t) = \sum_{t\in \T} w_t(c_t^S) =  \sum_{e\in E_{c^S}: e\subseteq S} w_e^{c^S}.$$
Now consider some vector $s$. We need to argue that $v(S) \geq \sum_{e\in E_c:e\subseteq S}w_e^{c}$. This follows from the fact that $v(S)$ is the sum of the values of completing each task in the best possible way, subject to having set $S$, while the right sum is the sum of tasks that can be completed by a specific combination, as long as this specific combination is a subset of $S$, which is always smaller.
\end{proof}}




==> hierarchies.tex <==
The proof of Proposition~\ref{prop:incompatible} is deferred to Section~\ref{sec:incompatible}. 


==> introduction_-_old.tex <==
% !TEX root=complements.tex

In a world with a diverse set of resources, individuals have complex valuations over potential allocations.  An indivdual in the market for a new laptop probably only desires one of the available resources (laptops in this case), whereas a company with a blitz advertising campaign may value an allocation only if it receives all available resources (ad spaces on a webpage, say).  Alternatively, an airline scheduling a flight from, say, Boston to Barbados, has no value for a takeoff slot without the corresponding landing slot (and vice versa), and also needs at most one of each resource (takeoff/landing slots in this case).  These valuations are of fundamentally different natures.  The individual buying a laptop has no extra value for multiple laptops; they are simply extraneous to him.  In this sense, one laptop is a {\it substitute} for another, i.e., he has {\it substitutable} values.  At the other extreme, the advertising company has zero value for any given ad slot unless it acquires every single ad slot in the market.  Here the ad slots {\it complement} each other in that the whole is worth more than the sum of the parts and we say the advertiser has {\it complementary} values.  The third setting is somewhat intermediary.  A particular takeoff slot complements a particular landing slot, but a pair of comlpementary takeoff/landing slots is a substitue for another complementary pair.

How should resources be be divided among parties in such complex settings?  This problem lies at the heart of much algorithmic and economic theory.  A long line of literature focuses on solving this problem for settings with substitutable valuations, providing algorithms and mechanisms that (approximately) optimize the total value, or {\it welfare}, generated by the allocation.  This literature defines a classification of substitutable valuations, first introduced by Lehmann, Lehmann, and Nisan~\cite{Lehmann2001}.  The approximation of the welfare maximization problem changes with respect to the class, but is at worst constant: the laptop allocation problem discussed above is a case of {\it unit demand} valuations and can be solved optimally; the more general cases of {\it submodular} valuations, {\it $\XOS$} valuations, and (most generally) {\it subadditive} valuations can be solved to within a ratio somewhat better than $1 - 1/e$~\cite{FV}, $1 - 1/e$~\cite{DS2006}, and~2~\cite{Feige2006} respectively.\footnote{These approximation algorithms assume {\em demand queries} access to the valuation functions, though for the submodular case, if one is satisfied with a $1 - 1/e$ ratio, then {\em value queries} suffice~\cite{Vondrak}.  See Appendix~\ref{app:poly-representation} for more details.}
These valuation classes have also been studied in the game-theoretic context of equilibria in simultaneous single-item auctions.  It has been established that the \emph{price of anarchy} (that is, the worst-case approximation over all equilibria) of this auction format, combined with a first-price payment rule, are at most $e/(e-1)$ for $\XOS$ valuations~\cite{Syrgkanis2012a} and~2 for subadditive valuations~\cite{Feldman2013}. %These results build upon a line of work studying non-truthful item auctions for complement-free valuations \cite{Bikhchandani1999,Bhawalkar2011,Christodoulou2008,Hassidim2011,PaesLeme2012}.


Complementary valuations, on the other hand, are significantly more complex.  For these valuations, optimizing the welfare can be as hard as solving independent set and is thus inapproximable (see, e.g.,~\cite{LCS99}).
As a result, much of the prior literature has focused on restricted classes of complementary valuations.
Some examples of these include the so-called {\em graphical valuations} introduced by Conitzer, Sandholm, and Santi~\cite{Conitzer2005}, in which the items are represented as vertices of a positively and negatively weighted graph and the value of a subset is the weight of the induced subgraph, and the hierarchy of valuations with pure complements called {\em positive hypergraph} ($\PH$) valuations, introduced by Abraham, Babaioff, Dughmi and Roughgarden~\cite{Abraham2012}, in which the items are vertices of a positively-weighted hypergraph and the value of a subset is the weight of the induced sub-hypergraph.
Another approach that has been studied by Feige and Izsak~\cite{Feige2013} is to define an hierarchy capturing any monotone valuation that admits approximation guarantees proportional to the level of the hierarchy the valuations belongs to.
Specifically, \cite{Feige2013} introduced the {\it supermodular degree} hierarchy and presented a $(k+2)$-approximation algorithm for welfare maximization with valuations that belong to level $k$ of the hierarchy (see also \cite{FeldmanIzsak2014} for a more general application of the supermodular degree).

\Omit{Two approaches to cope with this hardness that can be found in prior literature are restricting the valuations and using hierarchies of valuations, where the performance guarantee degrades with the hierarchy level.
An example for the first is the work of Abraham, Babaioff, Dughmi and Roughgarden~\cite{Abraham2012} who studied a hierarchy of valuations that captures only pure complements (we call it {\it positive hypergraph} ($\PH$) valuations).
An example for the latter is the work of Feige and Izsak~\cite{Feige2013} who introduced the {\it supermodular degree} hierarchy that captures any monotone set function. Both works present an algorithm for the welfare maximization problem (non truthful) with approximation guartantee linear in the lowest level of the respective hierarchy the valuations of the agents belong to.  
Unfortunately, although the supermodular degree captures any monotone set function, it captures some of the lowest levels of the $\PH$ hierarchy only by arbitrarily high levels of it (i.e. the level may depend on the number of items of the instance).

Each of these classifications has some compelling properties.  For instance, graphical valuations are compatible with natural, iterative auction designs~\cite{Acemoglu2012}. Algorithmically, welfare can be maximized for $\PH$-$k$ valuations (i.e., those at level $k$ of the $\PH$ hierarchy) to within $k$.
}
%As a result, much of the prior literature has focused on either restricted classes of complementary valuations or on hierarchies where the performance guarantee degrades with the hierarchy level.  Some examples of these include the so-called {\em graphical valuations} introduced by Conitzer, Sandholm, and Santi~\cite{Conitzer2005} in which the items are represented as vertices of a positively and negatively weighted graph and the value of a subset is the weight of the induced subgraph; the hierarchy of valuations with pure complements called {\em positive hypergraph} ($\PH$) valuations, introduced by Abraham, Babaioff, Dughmi and Roughgarden~\cite{Abraham2012} in which the items are vertices of a positively-weighted hypergraph and the value of a subset is the weight of the induced sub-hypergraph; and the {\it supermodular degree} hierarchy of Feige and Izsak~\cite{Feige2013} (defined in Section~\ref{sec:supermodular}).  

Each of these classifications has some compelling properties.  For instance, graphical valuations are compatible with natural, iterative auction designs~\cite{Acemoglu2012}. Algorithmically, welfare can be maximized for $\PH$-$k$ valuations (i.e., those at level $k$ of the $\PH$ hierarchy) to within $k$, and in supermodular of degree $k$ to within $k+2$.  However, these existing classifications have significant drawbacks.  Graphical valuations fail to capture valuations with ``large'' complementarities like the advertising example above; $\PH$-$k$ valuations fail to include valuations that have some substitutability like the takeoff/landing slot example above; and supermodular degree, while containing all monotone valuations, %does not distinguish among valuations sufficiently to leverage their approximability.  
contain some functions of the lowest levels of the $\PH$ hierarchy only in arbitrarily high levels of it.

\Omit{
There is a more expressive hierarchy that subsumes many of the hierarchies described; namely, the {\it hypergraph} hierarchy, which is similar to $\PH$-$k$ but allows both positive and negative hyperedge weights.  This natural classification generalizes both the $\PH$-$k$ hierarchy and graphical valuations.  However, this classification has not yet yielded natural algorithmic results.  This has necessitated the recent attention on more restrictive hierarchies, like the ones described above.
\ricomment{and it cannot even approximate the supermodular degree hierarchy}.
}

%Our work attempts to bridge the gap between expressive but algorithmically unweildy hierarchies, like the hypergraph hierarchy, and useful but less expressive hierarchies, like $\PH$-$k$.  
We introduce a new hierarchy, called {\em maximum over positive hypergraphs} ($\MOPH$), whose levels capture degree of complementarity.  Our hierarchy is general enough to encapsulate all monotone valuation functions.
Specifically, any graphical valuation belongs to level~2 of it. %, regardless of the number of items in the groundset.
It also compares favorably to the existing hierarchies of $\PH$-$k$ and supermodular degree $k$ in that every level of our hierarchy is a strict superset of the corresponding level of existing hierarchies.  In fact, to even approximate functions in low levels of our hierarchies, one must use functions from arbitrarily high levels of the existing hierarchies. \nicomment{REF TO CONJECTURE HERE?}  %For an extended discussion of related work, including a more formal development of the relationship between our work and prior literature, see Appendix~\ref{sec:related}.

%We complement our hierarchy with powerful 
We present algorithmic and economic results that illustrate the usefulness of our hierarchy.  We develop an algorithm that approximates the welfare maximization problem to within a factor of $k+1$, where $k$ is the level of the hierarchy the valuations belong to (i.e., degree of complementarity).  We further show that an auction that solicits separate bids on each item separately and allocates each item to the highest bidder (at a cost equal to the winning bid) attains a $2k$-approximation to the optimal welfare at any equilibrium of bidder behavior.  
%Finally, we conjecture that the set of $\MOPH$ hierarchy compares favorably with the very general hierarchy based on hypergraph rank; we present a number of intermediate results representing progress toward this conjecture.

The rest of our paper is organized as follows.  We formally define the concepts described above in Section \ref{sec:prelims}, and present our new valuation hierarchy in Section \ref{sec:moh}.  Then, in Section \ref{sec:results} we provide a more precise summary of our technical results.  In Section \ref{sec:connections} we establish the expressiveness of the $\MOPH$ hierarchy relative to other hierarchies from the literature, and explore the relationship between the $\MOPH$ hierarchy and general hypergraph rank.  In Section \ref{sec:welfare} we present our algorithmic and game theoretic results, establishing approximation algorithms and price of anarchy results for valuations in low levels of the $\MOPH$ hierarchy.  In Section \ref{sec:non-monotone} we discuss an extension of our hierarchy that also includes non-monotone valuations.

%OUTLINE OF PAPER HERE.  MOVE CURRENT RELATED WORK TO APPENDIX AND POINT TO IT HERE AS A MORE FORMAL DEVELOPMENT OF THE RELATIONSHIP BETWEEN OUR WORK AND PRIOR WORK.










\iffalse


How should resources be divided among individual parties, in order to optimize global efficiency?  This optimization problem lies at the center of algorithmic and economic theory, exhibiting both computational and incentive constraints.  A canonical instantiation of this problem is the
combinatorial auction setting, in which a set $M$ of $m$ indivisible goods is to be allocated among a set $N$ of $n$ buyers. Each buyer $i\in N$ has a valuation function that assigns a non-negative real number $v_i(S)$ to every bundle of goods $S\subseteq M$ . A well motivated objective is to find an allocation of the goods that maximizes the {\em social welfare}, defined as the sum of buyers' valuations from the bundles they obtain. The model of combinatorial auctions is highly applicable to real-world settings such as spectrum auctions and electronic advertisement markets.

For completely general valuations, the combinatorial auction problem is known to be highly inapproximable; for example, it subsumes the maximum independent set problem.
Thus, out of necessity, most of the existing literature on combinatorial auctions has focused on tractible special cases.  The class of complement-free valuations has led to an especially fruitful line of inquiry.
Roughly speaking, complement-freeness means that the value for the union of two bundles of items cannot exceed the sum of the values for each individual bundle.
Such valuations do not capture scenarios where certain goods produce more value when acquired in conjunction with each other (such as a left and right shoe).
Complement-free valuations are arguably more well-behaved than general combinatorial valuations in many aspects.
From an algorithmic perspective, complement-free valuations admit constant-factor polynomial time approximation algorithms (see for example \cite{Lehmann2001, DNS, Feige2006}), while general valuations are hard to approximate even to within a factor that is sub-polynomial in the number of items \cite{NS2006}.
From a game-theoretic perspective, simple auctions, such as running simultaneously a single-item first-price auction for each item, induce equilibria that achieve constant factor approximations to the optimal welfare if all valuations are complement-free \cite{STOC13}. In contrast, if valuations exhibit complements, the inefficiency can grow with the number of items \cite{Hassidim11}.

While the theory suggests that complementary relations degrades the performance of combinatorial auctions, complementarity arises very naturally in many economic scenarios. A prominent example is the FCC spectrum auctions, where it is desirable to win licenses for the same band of spectrum in adjacent geographical regions. The prevalence of complementarities in practice calls for a better theoretical understanding of general valuation functions.
Ideally, we aim to introduce a meaningful measure for the degree of complementarity that will capture well the effect of complementarities on different performance measures.

%\ricomment{should be rephrased. On one hand ``we introduce a new *hierarchy*'' and on the other ``We refer to this *class*''.}
To this end, we introduce a new hierarchy of valuation classes that includes all monotone set functions.
We refer to the $k^{\text{th}}$ class in this hierarchy as {\em Maximum over Positive Hypergraphs} of degree $k$ ($\MOPH$-$k$), where $k \geq 1$ is a parameter reflecting the degree of complementarity.
This class is syntactic; it is based on the class of Positive Hypergraph-$k$ ($\PH$-$k$) functions, introduced by Abraham, Babaioff, Dughmi and Roughgarden \cite{Abraham}.
A function $v$ is $\PH$-$k$ if it has a positive hypergraph representation with rank $k$; i.e., a function $h$ that assigns a non-negative value to every subset $T$ of size up to $k$, such that $v(S)=\sum_{T \subseteq S}h(T)$ for every set $S$.
A subset with a strictly positive value is referred to as a hyperedge, and the size of the largest hyperedge is called the rank of $h$.
A set function is $\MOPH$-$k$ if it can be expressed as a maximum over an arbitrary set of $\PH$-$k$ functions.
%$\MOPH$ is a general hierarchy over set functions.
%\ricomment{omitted: ``$\MOPH$ is a general hierarchy over set function''. We've just said that (in this paragraph). Additionally, if we do want to say it again, I think we have to say ``monotone set functions''.}
In this paper we focus on the applications of this hierarchy to combinatorial auctions.

%\subsection{Our results}
%
%We obtain results on the expressiveness power of the $\MOPH$-$k$ hierarchy and on the approximability of social welfare in combinatorial auctions with $\MOPH$-$k$ valuations, from both algorithmic and game-theoretic perspectives.
%%
%The first theorem establishes the expressiveness power of our hierarchy.
%
%\begin{theorem} \label{t:expressiveness} \label{thm:expressiveness}
%The $\MOPH$ hierarchy captures many existing hierarchies, as follows:
%\begin{enumerate}
%\item The class $\MOPH$-$1$ is, by definition, equivalent to the class $\XOS$ (in the sense defined by Lehmann, Lehmann and Nisan \cite{Lehmann2001}).
%
%\item Every monotone graphical valuation (in the sense defined by Acemoglu et al. \cite{Acemoglu2012}) is in $\MOPH$-2 (see Section~\ref{}). Furthermore, every monotone function with positive rank~2 is $\MOPH$-2.
%
%\ricomment{I'm not sure about the reference. Have they been the first ever to consider graphical valuations? I think it was studied years before. Wasn't it?}
%\ricomment{I'd consider adding here a furthermore clause for arbitrary negative edges.}
%\blcomment{Note also that ``positive rank'' hasn't yet been defined.}
%
%\item Every function that has a positive hypergraph representation of rank $k$ (in the sense defined by Abraham et al. \cite{Abraham2012}, see Section~\ref{}) is, by definition, in $\MOPH$-$k$.
%
%\Omit{\item Every monotone function that has a hypergraph representation with positive rank $k$ and laminar negative hyperedges (with arbitrary rank) is in $\MOPH$-$k$ (See Section~\ref{}).}
%\ricomment{We haven't defined yet positive rank. Moreover, I don't think it is a well known notion. It is better to define it before this theorem, or at least to add a reference to preliminaries (better to define before, if flows).}
%\ricomment{We can consider adding here a comparison to ABDR (i.e. to $\PH$-$k$). Can also move this item to be a furthermore clause for $\PH$-$k$. This way we have one item less and we also emphasize we have strictly more than ABDR in the same item. In any case, I put it right after the $\PH$-$k$ item.}
%
%\blcomment{I'd actually propose not mentioning this item; it seems out of place since the other items are classes considered elsewhere.  Instead, we could pose our conjecture that hypergraph representations can be captured by our hierarchy, and state that we establish this for certain rich subclasses that we'll define later, with a forward pointer to the appropriate section.}
%
%\item Every monotone function that has supermodular degree $k$ (in the sense defined by Feige and Izsak \cite{Feige2013}) is in $\MOPH$-$(k+1)$ (See Section~\ref{}).
%%%\item Every function that can be represented as XOR of ORs of bundles of size $k$ (as defined by Sandhold \cite{}) is in $\MOPH$-$k$ (See Section~\ref{}).
%
%\end{enumerate}
%\end{theorem}
%%\ricomment{I think we should consider an alternative wording for the following 2 sentences (limitations seems problematic to me).}
%%The introduction of a new hierarchy is desired, in part, due to the limitations of previous hierarchies.
%%To demonstrate these limitations, we define the following notion of approximation:
%
%We further establish that the converse direction does not hold, not even in an approximate sense, and conclude that 
%the $\MOPH$-$k$ hierarchy is \emph{strictly} more expressive than many existing hierarchies.  
%Specifically, we show that $\MOPH$-$1$ and $\MOPH$-$2$ contain functions that cannot be \emph{approximated} by functions in low levels of other hierarchies.
%Before stating the result, we define the notion of approximation.
%
%\begin{defn} \label{def:approximate}
%\label{def:approximation}
%We say that a set function $f$ approximates a set function $g$ within a ratio of $\rho \ge 1$ if there are $\rho_1$ and $\rho_2$ such that for every set $S$
%$\rho_1 \le \frac{f(S)}{g(S)} \le \rho_2$, and $\frac{\rho_2}{\rho_1} \le \rho$.
%\end{defn}
%
%
%%The following proposition shows that the previous hierarchies are mutually incomparable in the sense of the above definition.
%%These results are discussed in Section~\ref{}).
%
%\blcomment{Rather than describe the issue as ``incompatibility'' in the statement of Proposition \ref{prop:incompatible}, could we instead state the proposition as establishing that $\MOPH$ is strictly more expressive than many existing hierarchies, even with respect to approximation?  This would make it clear that Proposition \ref{prop:incompatible} is about $\MOPH$, rather than being about the space of hierarchies more generally.}
%
%We are now ready to state the proposition. Its proof is deferred to Appendix~\ref{app:incompatible}.
%
%
%\begin{prop} \label{prop:incompatible}
%Previous hierarchies are mutually incompatible in the sense that functions in very low levels of one hierarchy cannot be approximated well even at relatively high levels of other hierarchies.
%\begin{enumerate}
%\item There exists a submodular function (i.e., supermodular degree $0$, $\MOPH$-$1$) such that
%\begin{enumerate}
%\item A graphical function cannot approximate it within a ratio better than $\Omega(m)$.
%\item A positive hypergraph function cannot approximate it within a ratio better than $m$.
%\item A hypergraph function of rank $k$ (both negative and positive) cannot approximate it within a ratio better than $\Omega{\frac{m}{k^2}}$, for every $k$.
%\end{enumerate}
%\item There exists a $\PH$-2 function (i.e., $\MOPH$-2) such that every function of supermodular degree $d$ cannot approximate it within a ratio better than $\Omega(m/d)$.
%\end{enumerate}
%\end{prop}
%
%With the new hierarchy at hand, we are in a position to revisit fundamental algorithmic and game-theoretic problems about welfare maximization in combinatorial auctions.
%Our results are reassuring: we obtain good approximation ratios for settings with valuations that lie in low levels of the $\MOPH$-$k$ hierarchy.
%From the algorithmic perspective, we provide a polynomial time $(k+1)$-approximation algorithm for the welfare maximization problem when valuations are $\MOPH-k$ (assuming an access to a demand oracle).
%
%%\ricomment{I added a label. Should be referenced also from the section. Perhaps also the same for the first theorem.}
%\begin{theorem} \label{t:algorithmic}
%If all agents have $\MOPH$-$k$ valuations, then there exists an algorithm that gives $k+1$ approximation to the optimal social welfare.
%This algorithm runs in polynomial time given an access to demand oracles for the valuations.
%\end{theorem}
%
%Our approximation algorithm first solves the configuration linear program for welfare maximization introduced by \cite{DNS}.
%As is well known, solving this LP can be done in polynomial time using demand queries.
%\ricomment{I think it might be problematic to call it new, if it was used to solve other problems.
%Perhaps better to say something like: ``we observe that rounding by a random permutation on the players gives approximation guarantee which is at least nearly best possible for this LP. This is shown by upper bounding the approximation guarantee and lower bounding the integrality gap.''}
%We then resolve conflicts using a new contention resolution algorithm, to account for complementarities.
%By analyzing the integrality gap, it is established that our rounding technique is nearly best possible.
%
%The second setting we consider is a simultaneous first-price auction --- where each of the $m$ items is sold via a separate single-item auction.
%We quantify the welfare loss in this simple auction when bidders have $\MOPH$-$k$ valuations.
%%\ricomment{If it's $2k$, I think it is better to just say it.}
%We find that the price of anarchy is at most $2k$.
%
%\begin{theorem} \label{t:poa}
%For simultaneous first price auctions, when bidders have $\MOPH$-$k$ valuations, both the correlated price of anarchy and the Bayes-Nash price of anarchy are at most $2k$.
%\end{theorem}
%
%Our proof technique extends the analysis for complement-free valuations in \cite{Feldman2013} and the smoothness framework introduced in \cite{Syrgkanis2013} to settings with complementarities.
%
%\paragraph{Extensions}
%%\ricomment{I'd prefer changing the word ``left'' to something more like ''suggested by this work''.}
%One of the main open problems suggested by this work is the relation between hypergraph valuations of rank $k$ and $\MOPH$-$k$ valuations.
%We make the following conjecture:
%\begin{conj} \label{conj:quadratic}
%Every hypergraph function with rank $k$ (positive or negative) is in $\MOPH$-$O(k^2)$.
%\end{conj}
%We make partial progress toward the proof of this conjecture.
%For $k=2$ this conjecture is confirmed in Theorem~\ref{}, whose proof is based on flow arguments.
%This conjecture is also confirmed for the special case of symmetric functions, for any $k$, using Markov inequalities on derivatives of polynomials (See Section~\ref{}).
%For symmetric functions, we actually conjecture a more precise bound of $\left\lceil \frac{r}{2} \right\rceil \left\lceil \frac{r+1}{2} \right\rceil$, which is suggested by a computer-assisted simulation based on a non-trivial LP formulation.
%\ricomment{TODO (Rani): add here a few words about the technique.}
%For the special cases of hypergraph functions of ranks $k=3$ and $k=4$, we show analytically that they are in $\MOPH$-4 and $\MOPH$-6, respectively, and that this is tight.  \blcomment{TODO: say a few words about hypergraph valuations with laminar negative edges}
%
%Most of our expressiveness results showing that a certain function belongs to $\MOPH$-$k$ are established by showing that the function satisfies a certain requirement that we refer to as the Positive Lower Envelope (PLE) condition.
%We also observe that, together with monotonicity, this requirement becomes a sufficient and necessary condition for membership in $\MOPH$-$k$.
%This observation motivates the definition of a new hierarchy, referred to as $\PLE$.  The class $\PLE$-$k$ contains $\MOPH$-$k$, but also includes non-monotone functions.
%%but without the monotonicity requirement.
%%\ricomment{Is it accurate?}
%Our approximation results in Theorems~\ref{} and~\ref{} carry over to $\PLE$-$k$ functions, assuming that goods are allowed to remain unallocated.
%Exploring the relations between the expressiveness of hypergraph valuations and the $\PLE$ hierarchy is a fertile ground for future research.
%See Section~\ref{} for some preliminary results.
%It should be noted that while monotonicity is a standard assumption in the context of combinatorial auctions, this class can be highly applicable outside the scope of combinatorial auctions.


\fi


==> moh-old.tex <==
In this section we introduce the class of Maximum over Hypergraph-$k$ (MOPH-$k$) valuations.  This class of valuations is a generalization of both submodular valuations and positive hypergraph-$k$ valuations, and further permits both substitute and restricted complementary relations among different items.

A {\em hypergraph representation} $h$ of a valuation (set) function $v$ is a set function that satisfies $v(S) = \sum_{T \subset S} h(T)$ (in our notation, containment of sets need not be strict, namely $T \subset T$ holds).
We also refer to $h(S)$ as the weight of $S$.
It is easy to verify that given $h$, the corresponding $v$ is uniquely determined, and vice versa.
The {\em rank} of $h$ is the largest cardinality $r$ such that there is a set $S$ with $|S| = r$ and $h(S) \not=0$.
The rank of $v$ is the rank of its corresponding $h$.
A set $S$ such that $h(S)\neq0$ is said to be a hyperedge of $h$, or simply an edge of $h$.
The set of edges of $h$ is denoted by $E_h$, or simply $E$ when clear in the context.
The set of edges that are subsets of a set $S$ and have cardinality up to $k$ is denoted by $S|_k$.
The set of edges of a valuation $v$ is the set of hyperedges of its corresponding hypergraph representation.

A hypergraph representation is {\em positive} if $h(S) \ge 0$ for every $S$.
The function $h$ is a hypergraph-$k$ representation if $h$ is positive and has rank $k$.
The valuation $v$ is hypergraph-$k$ if its corresponding hypergraph representation is hypergraph-$k$.
A special case of hypergraph-$k$ valuations is that of hypergraph-$2$ valuations, which correspond to the set of graphical valuations with non-negative weights (see e.g., \cite{Acemoglu2012}).

Intuitively, hyperedges in hypergraph-$k$ valuations correspond to groups of items that exhibit complementarities, and the edge's weight is the added value when consuming all the items in the group.
While hypergraph-$k$ valuations capture $k$-wise complements, they are not expressive enough to capture substitute relations.
Even simple classes of valuations such as unit-demand valuations cannot be expressed by hypergraph-$k$ valuations.
This limited expressiveness motivates us to introduce a new class of valuations that captures $k$-wise complements but also substitute relations.

\begin{defn}[Maximum Over Hypergraph-$k$]
A monotone valuation $v$ is {\em maximum over hypergraph-$k$} (MOPH-$k$) if it can be expressed as a maximum over a set of hypergraph-$k$ valuations.  That is, there exist hypergraph-$k$ valuations $\{v^{\ell}\}_{\ell\in\Ell}$ such that for every set $S \subset [m]$,
\begin{equation}
\textstyle{v(S) = \max_{\ell \in \Ell} v^{\ell}(S) = \max_{\ell\in \Ell}\sum_{s\in \ESk{S}} w_s^{\ell}}
\end{equation}
where $\Ell$ is an arbitrary index set and $w_s^{\ell}\geq 0$ for each $\ell\in\Ell$ and $s\in\ESk{S}$.
\end{defn}

For $k=1$ the latter definition coincides with the class of $XOS$ valuations, a complement-free class of valuations that contains all submodular valuations.
For $k=m$, it coincides with the class of monotone valuations\footnote{Simply create a separate hypergraph-$m$ valuation for each set $S$ with a single hyperedge equal to the set $S$ and with weight $v(S)$. Then by monotonicity the maximum of these hypergraph valuations is equal to the initial valuation.}.
For intermediate values it holds that for every $k< k'<m$, $\text{MOPH-}k\subset \text{MOPH-}k'$.
We get the following hierarchy:
\begin{equation}
\text{Submodular}\subset XOS \equiv \text{MOPH-}1 \subset \text{MOPH-}k'\subset \text{MOPH-}k\subset \text{MOPH-}m\equiv \text{Monotone}
\end{equation}
We defer some deeper insights on the expressiveness of MOPH-$k$ valuations to Section \ref{sec:connections}.



%A set function is symmetric if $f(S) = f(T)$ whenever $|S| = |T|$.
%Given $h$, the corresponding $v$ is uniquely determined, and vice versa.
%It follows that if $f$ is symmetric, so is its hypergraph representation, and vice versa.



%A (positively) weighted hypergraph defines a valuation function as follows: items are nodes and the value of a subset of items is the total weight of the hypergraph induced on the nodes representing those items.  The valuation thus obtained is a {\it hypergraph-$k$ valuation} if the hyperedges have size at most $k$.  Conversely, a valuation is a hypergraph-$k$ valuation if it can be written in this form.  More formally, let $\ESk{S}$ denote the collection of all subsets of size at most $k$, of a given set $S$.

%\begin{defn}
%A monotone valuation $v$ on a set $[m]$ of items is {\em hypergraph-$k$} if there exist weights $w_s\geq0$ such that for any set $S\subseteq [m]$: $v(S) = \sum_{s\in \ESk{S}} w_s$. A {\em hyperedge} of the valuation is a set $s\in \ESk{[m]}$ of strictly positive weight. The set of all hyperedges of a valuation will be denoted by $E$.
%\end{defn}


==> non-monotone.tex <==
% !TEX root=complements.tex

As we saw in Section \ref{sec:proofs}, positive lower envelopes are a useful tool for showing that a monotone function admits a $\MOPH$-$k$ representation. Observe that while $\MOPH$-$k$ contains only monotone functions, even a non-monotone function can admit a positive lower envelope for any restriction to a subset. %The catch being that now we can no-longer claim that it is also $\MOPH$-$k$.
This observation motivates the following hierarchy of (not necessarily monotone) set functions.
%, that goes beyond monotone functions, to the whole class of non-negative functions. Though monotonicity is a very natural assumption in the context of combinatorial auctions, and hence the reason why we focused on them in the main part of the paper, analyzing hierarchies of non-monotone functions can have potential applications in contexts outside of the combinatorial auction setting, such us set function minimization and maximization.

\begin{defn} [Positive Lower Envelope $k$ ($\PLE$-$k$) class]
Let $f: 2^M \to \nonnegR$ be a set function.
$f$ is in $\PLE$-$k$ if any restriction of it to a subset of its ground set admits a positive lower envelope of rank $k$.
\end{defn}

While monotonicity is a very natural assumption in the context of combinatorial auctions, %and hence the reason why we focused on them in the main part of the paper,
hierarchies of non-monotone functions can have potential applications in more general contexts
%outside of the combinatorial auction setting,
such as set function minimization and maximization.

In Propositions~\ref{p:PLEtoMOH} and~\ref{p:MOHtoPLE} we showed that $\PLE$-$k$ is equivalent to $\MOPH$-$k$ for monotone functions.
%Moreover, it is easy to see that if a function is $\MOPH$-$k$, then it is also $\PLE$-$k$.
Thus $\MOPH$-$k$ is exactly the monotone part of the $\PLE$-$k$ class. Moreover, we point out that both our algorithmic approximation result (Theorem~\ref{t:algorithmic}) and our price of anarchy result (Theorem~\ref{t:poa}) apply more generally to the class of $\PLE$-$k$ functions, and in particular do not require monotonicity (assuming that players are able to drop out of an auction and receive no items).

With respect to expressiveness, exploring the expressive power of the $\PLE$ hierarchy is an interesting space for future research. In particular, one might explore the connection between $\PLE$-$k$ and the class of functions with a given positive and/or negative hypergraph rank.  %and the positive and negative rank of a function is also a very interesting space for future research.
To this end, we show some results on this connection.
%We show some characterization regarding this connection.
We first observe that a strong positive result similar to Theorem \ref{t:PleForAnyMonotoneSymmetricFunction},
cannot possibly hold for non-monotone non-symmetric set functions.
That is, for any constant $k$, there exist a non-negative set function of rank $2$ that is not $\PLE$-$k$. 
%(see Appendix \ref{sec:app-non-monotone}). 

This is not the case for non-negative functions with positive rank $1$ and arbitrary negative rank, which can be shown to be in $\PLE$-$1$.
%(see Appendix \ref{sec:app-non-monotone}). %Moreover, if one assumes some structure on the hypergraph representation, such as that the negative hyperedges form a laminar family, then we easily observe that


Moreover, the proof of Theorem~\ref{t:laminar_nonneg} extends to non-negative functions in $\PLE$-$k$. That is, any non-negative function with positive rank $k$ and arbitrary negative rank is in $\PLE$-$k$, if negative hyperedges are laminar.



%\begin{prop} \label{p:MOHtoPLE}
%Any function that is $\MOPH$-$r$ is monotone and has positive lower envelope for any restriction of it to a subset of its groundset.
%\end{prop}
%
%
%\begin{proof}
%Let $f: 2^M \to \nonnegR$ be a function that is $\MOPH$-$r$.
%We show monotonicity. Assume towards a contradiction that $f$ is not monotone.
%Then, there exist $S' \subset S \subseteq M$ such that $f(S') > f(S)$.
%Therefore, in any $\MOPH$ representation of $f$, there exists a positive hypergraph such that $S'$ gets value $f(S')$ according to it.
%But, this means that $S$ also gets at least value $f(S')$ by this positive hypergraph. Therefore, $S'$ gets at least value $f(S') > f(S)$ by any $\MOPH$ representation of $f$. contradiction.
%Therefore, $f$ must be monotone.
%We show existence of positive lower envelope for $f$ for any restriction of it to a subset of its groundset.
%Let $S \subseteq M$ and let $F$ be an $\MOPH$-$r$ representation of $f$.
%Then, there exists a positive hypergraph $H$ in $F$ such that $S$ gets value $f(S)$ according to it.
%Moreover, any subset $S' \subseteq S$ cannot get value of more than $f(S')$ according to it since then this will be a lower bound on its value according to $F$.
%Therefore $H$ is a positive lower envelope of $f$ restricted to $S$, as desired.
%We conclude the proof of Proposition~\ref{p:MOHtoPLE}.
%\end{proof}
%
%Let $k',k \in \mathbb{N}$ be such that $k' < k$.
%Since it is trivial that any function has a positive lower envelope of rank $t$ for any subset of cardinality $t$,
%we have the following hierarchy\footnote{simply take as the hypergraph representation of the positive lower envelope a graph with one hyperedge of rank $t$ that has value as the value of the subset by the function.}.
%\begin{equation} \label{eq:ple_hierarchy}
%\MOPH\text{-}k' \subset \PLE\text{-}k'\subset \PLE\text{-}k\subset \PLE\text{-}m = \text{Non-negative}
%\end{equation}
%Note that as for $\MOPH$, an immediate consequence of Equation~\eqref{eq:ple_hierarchy} is that $\PLE$ can be used as a complexity measure for any {\em non-negative} (i.e. and not necessarily monotone) set function.
%
%
%\subsection{A characterization of non-negative non-laminar set functions} 

==> old-abstract.tex <==
\Omit{We propose a new class of valuations that allows for the expression of both substitute and restricted complementary relations across goods. Specifically, we propose the class of valuations that can be expressed as the maximum over a set of positive hypergraph values with restricted edge-size, and can be thought as a generalization of fractionally subadditive valuations. For the given class we address expressiveness, algorithmic and price of anarchy questions. We show that such valuations generalizes various notions of restricted complementarities, including supermodular degree recently introduced by Feige and Izsak \cite{Feige2013}, hypergraph valuations \cite{Abraham2012}, as well as monotone graphical valuations with positive and negative weights \cite{Acemoglu2012}. We show that the price of anarchy of simultaneous first-price item auctions is at most $2k$, where $k$ describes the degree of complementarity. Our analysis proceeds via the smoothness framework, and therefore also applies to Bayesian equilibria and learning outcomes. Finally, we extend our results to the simultaneous composition of smooth mechanisms (e.g. simultaneous position auctions) under valuations that allow for restricted complements across mechanisms.}


==> old-file.tex <==
\begin{proofof} {Proposition~\ref{p:PLEtoMOH}}
Let $f:2^M \to \nonnegR$ be a monotone set function.
For any $T \subseteq M$, let $g_T$ be a positive lower envelope of rank $k$ of $f$ restricted to $T$.
We argue that $\{g_T\}_{T \subseteq M}$ is a $\MOPH$-$k$ representation of $f$.
%Firstly, it is clear that all these hypergraph functions are positive and have rank up to $k$.
%Firstly, it is clear this is a legal $\MOPH$-$k$ representation.
Specifically, we show that for every $S \subseteq M$, it holds that $\max_{T \subseteq M} g_T(S) = f(S)$.
Let $S \subseteq M$.
By the no-underestimate property of Definition~\ref{def:PLE}, it holds that $g_S(S) = f(S)$.
Therefore,
\begin{equation} \label{appPle:eq:nounderestimate}
\max_{T \subseteq M} g_T(S) \geq g_S(S) \geq f(S)
\end{equation}
Additionally, for any $T \subseteq M$, $g_T(S) = g_T(S \cap T) \leq f(S \cap T) \leq f(S)$,
where the equality follows from the fact that $g_T$ is restricted to $T$; the first inequality follows from the no-overestimate property of Definition~\ref{def:PLE} and the last inequality follows from monotonicity of $f$.
Therefore,
\begin{equation} \label{appPle:eq:nooverestimate}
\max_{T \subseteq M} g_T(S) \leq f(S)
\end{equation}
The proof of Proposition~\ref{p:PLEtoMOH} follows from~\eqref{appPle:eq:nounderestimate} and~\eqref{appPle:eq:nooverestimate}.
\end{proofof}

\noindent\begin{proofof} {Proposition~\ref{p:MOHtoPLE}}
Let $f: 2^M \to \nonnegR$ be a function in $\MOPH$-$k$ and let $\Ell$ be an $\MOPH$ representation of it.
We first prove that $f$ is monotone.
Assume towards a contradiction that $f$ is not monotone.
Then, there exist $S' \subset S \subseteq M$ such that $f(S') > f(S)$.
By the Therefore, there exists a positive hypergraph function $f_h \in \Ell$ such that $f_h(S')=f(S')$.
This means that $f_h(S) \geq f(S') > f(S)$. But, then $\max_{g \in \Ell} g(S) > f(S)$. contradiction.
%Therefore, $S'$ gets at least value $f(S') > f(S)$ by any $\MOPH$ representation of $f$. contradiction.
Therefore, $f$ must be monotone.
We show existence of positive lower envelope of $f$ of rank $k$, for any restriction of it to a subset of its groundset.
Let $S \subseteq M$. %and let $\Ell$ be a $\MOPH$-$k$ representation of $f$.
Then, there exists a positive hypergraph function $f_h \in \Ell$ such that $f_h(S)=f(S)$.
Moreover, any subset $S' \subseteq S$ cannot get value of more than $f(S')$ according to $f_h$ since then this will be a lower bound on the value of $S'$ according to $\Ell$.
Therefore $f_h$ is a positive lower envelope of $f$ restricted to $S$, as desired.
The proof of Proposition~\ref{p:MOHtoPLE} follows.
\end{proofof}

\Omit{
\begin{prop}
Every monotone set function is in $\MOPH$-$k$ if and only if every set $S \subseteq M$ admits a positive lower envelope of rank $k$.
\end{prop}


Before stating the formal theorem, we need the following preparation.
A set function $f:2^M\to \nonnegR$ restricted to a set $S\subset M$ is defined as $f_S:2^S\to \nonnegR$ with $f_S(T)=f(T)$ for any $T\subseteq S$. We show that if for every set $S \subseteq M$, the function restricted to $S$ admits a positive lower envelope of rank $r$, then the function admits an $\MOPH$-$r$ representation.

\begin{prop} \label{p:PLEtoMOH}\label{lem:lower-envelope}
Any monotone set function that has a positive lower envelope of rank $r$ for any restriction of it to a subset of its ground set is $\MOPH$-$r$.
\end{prop}

\begin{proofof} {Proposition~\ref{p:PLEtoMOH}}
Let $f:2^M \to \nonnegR$ be a monotone set function.
For any $S \subseteq M$, let $g_S$ be a positive lower envelope for $f$ restricted to items in $S$.
We argue that the collection of hypergraph representations $\{g_S\}_{S \subseteq M}$ is an $\MOPH$-$r$ representation of $f$ (that is $f(T)=\max_{S\subseteq M}g_S(T)$). Firstly, it is clear that all such hypergraph representations have rank up to $r$ and only positive hyperedges. Thus, this is a legal $\MOPH$-$r$ representation.
For the latter statement, it suffices to show that for any $S,T \subseteq M$, $f(T)\geq g_S(T)$ and $f(T)=g_T(T)$. The latter follows immediately by the second property of a positive lower envelope.
The former follows by monotonicity of $f$ and by the first property of a positive lower envelope.
Specifically, by monotonicity, $f(T)\geq f(T\cap S)$. By the positive lower envelope definition and the fact that $g_S$ spans only items in $S$, $f(T\cap S)\geq g_S(T\cap S)=g_S(T)$.
%Then, by definition of positive lower envelope, $g_S(S) = f(S)$.
%Additionally, by monotonicity, for any $S' \subset S$, $f(S') \leq f(S)$ and by the definition of positive lower envelope, it cannot be more than its original value by any function in $\{g_S\}_{S \subseteq M}$.
%We conclude the proof of Proposition~\ref{p:PLEtoMOH}.
\end{proofof}
}

\ricomment{in the appendix it seems to me redundant. If we want to state it, I think we should do it in the main text.}
\Omit{
Proposition~\ref{p:PLEtoMOH}, implies that we can use positive lower envelopes in order to prove a given set function is in $\MOPH$-$k$.
Moreover, the classes of set functions we consider are closed under restriction: i.e. if a set function $f: 2^M \to \nonnegR$ is in $\mathcal{C}$, then for any subset $S\subseteq M$, the restriction of $f$ to $S$: $f_S:2^S\to\nonnegR$, is also in $\mathcal{C}$.
This means that in order to prove membership of a class of functions in $\MOPH$-$k$ for some $k \in \mathbb{N}$, it is sufficient to prove existence of positive lower envelope of rank $k$ for each set function in the class without restricting it.
}


==> old-structure.tex <==
\Omit{Structure:
\begin{itemize}
\item In combinatorial auctions, agents have general valuations.
\item Roughly speaking, the literature can be divided into valuations encompassing substitutes and those exhibiting complements.
\item In many aspects, substitutes are "easier" than complements.
\begin{itemize}
     \item e.g., maximizing social welfare is computationaly "easy" with substitutes but "hard" with complements.
     \item e.g., simple auctions such as simultaneous first price auctions admit constant price of anarchy with substitutes but large POA for complements.
\end{itemize}
\item Goal: gain a better understanding of complements. What drives the negative results?
Can the negative results be mitigated under restricted complements?
\item To this end, we introduce a new class of valuations, that encompass both substitutes and complements,
but allows only a limited degree of complementarity. Our class is parameterized by the level of complementarity.
\item This enables us to study the problems above under restricted complements.
\item We study:
\begin{itemize}
\item the expressiveness of the introduced class.
\item social welfare approximation.
\item POA of simple auctions.
\end{itemize}
\end{itemize}}

==> omitted_text_before_SODA.tex <==
moh.tex (characterization):
A collection of subsets $\mathcal{T}$, together with a coefficient $a_T$ for any $T\in \mathcal{T}$, is a fractional cover of all the subsets of size at most $k$ ({\it $k$-fractional cover}) of a set $S$, if for any $S'\subseteq S$ with $|S'|\leq k$: $\sum_{T\supseteq S'} a_T\geq 1$. Then a set function is {\em $k$-fractionally subadditive} if $f(S) \leq \sum_{T\in \mathcal{T}}a_T f(T)$ for every $S$ and every $k$-fractional cover of $S$. Feige \cite{Feige2006} showed that the complement-free class of $\XOS$ valuations is equal to the class of $1$-fractionally subadditive functions.  A similar analysis shows that, for all $k$, the class of $\MOPH$-$k$ valuations equals the class of $k$-fractionally subadditive functions (see Appendix~\ref{sec:fractionally-subadditive}).  As was the case for $\XOS$ valuations, this alternate characterization may prove useful for deriving algorithms and mechanisms using linear programming techniques.

algorithmic-merged.tex (Solving the LP):
: i.e., the input to a demand query is ``prices'' $p_j$ for items $j\in M$, and an output is a subset of items $S\subseteq M$ maximizing $v_i(S)-\sum_{j\in S}p_j$. A known caveat regarding this approach is that answering a demand query might be $\NP$-hard in some cases. This issue is discussed in previous work, and we briefly present two ways by which it is mitigated. One is that in the context of combinatorial auctions, it is natural to expect the agent holding the valuation function to be able to answer demand queries (and hence to serve as a demand oracle) -- if agents do not know what they want to buy given a set of prices, it is somewhat unreasonable to expect the auction mechanism to allocate the agents the bundles that they want. The other involves the design of polynomial time algorithms for answering demand queries in cases of interest.  For $\MOPH$-$k$ valuations, if the valuation is supported on polynomially many positive hypergraphs, and each hypergraph has polynomially many edges, then a demand query can be answered in polynomial time. For further discussion, see Appendix~\ref{app:poly-representation}. 

==> poa-old.tex <==
[Place Holder for PoA. Other text is omitted below (i.e., with Omit command)]


\Omit{
% !TeX root = complements.tex

In this section we turn to a game-theoretic notion of welfare optimization.  We will bound the welfare loss at
equilibria of the simultaneous single-item auction, when all agents have $\MOPH$-$k$ valuations.
In a simultaneous (first-price) single-item auction, %each of the $m$ items is sold via a separate single-item auction.
%Formally, 
each bidder $i$ simultaneously submits a bid $b_{ij} \geq 0$ for each item $j$.
We write $b_i=(b_{i1},\ldots,b_{im})$ for the vector of bids from bidder $i$, and $b=(b_1, \ldots, b_n)$ for the bid profile.
The allocation and payments are determined separately for each item.
Each item is allocated to the bidder who bid highest on it (breaking ties arbitrarily),
and the winning bidder pays his bid.
%The allocation $X$ and payment $p$ are thus a function of the bids $b$.
We write $X_i(b)$ for the set allocated to bidder $i$ under bid profile $b$.
A bidders's utility %under a bid profile $b$ 
is assumed to be quasilinear in his allocation and his payment:
%\begin{equation}
$u_i(b;v_i)  = v_i(X_i(b))-\sum_{j\in X_i(b)}b_{ij}$. %, where $X_i(b)$ is the set allocated to bidder $i$.
%\end{equation}
% BJL: Removed the next sentence, since it is implied for first- and second-price simultaneous item auctions.  (We should state it when describing the more general results).
%We assume that a bidder always has the option to bid zero and drop out of the auction, resulting in a utility of $0$.
We also consider the case of a second-price auction, where the allocation rule is identical, but for each item the winning bidder pays the second-highest bid.

\paragraph{Solution Concepts and Price of Anarchy.}
We will quantify the efficiency\footnote{Throughout this section we use the term ``efficient" in the economic sense of ``optimizing social welfare.''} of the simultaneous auctions using the \emph{price of anarchy} measure, for both complete and incomplete information settings.  That is, we will bound the welfare obtained in the worst case over all equilibria of the auction.  Given a profile of valuations $\vals$, the social welfare (or efficiency) of an allocation $X$ is the sum of the agents' valuations: $SW(X;\vals)=\sum_{i=1}^{n}\val_i(X_i)$; we let $\opt(\vals)$ denote the social welfare of the optimal (welfare-maximizing) allocation.


For the complete information setting, our results will apply to the set of coarse correlated equilibria.  A joint distribution of bids $B$ constitutes a \textit{coarse correlated equilibrium} (CCE) if, for every player $i$ and for any bid $b_i'$,
\begin{equation}
\textstyle{\E_{\rbid\sim B}[u_i(\rbid;\val_i)]\geq \E_{\rbid\sim B}[u_i(\rbid_i',\rbid_{-i};\val_i)].}
\end{equation}
The \emph{correlated price of anarchy} is then defined to be the worst case approximation over CCEs:
\begin{equation}
POA = \max_{B \colon B \text{~is~} CCE} \frac{\opt(\vals)}{\E_{\rbid\sim B}[SW(X(\rbid))]}.
\end{equation}
We note that the set of CCE also includes all pure, mixed, and correlated Nash equilibria.  Our upper bounds on PoA therefore also apply to these equilibrium concepts.  Furthermore, the set of CCE is known to coincide with the limit of empirical distributions of no-regret repeated game-playing, and hence our bounds also apply to such learning outcomes.

% the valuation profile $v$ is common knowledge among the bidders, and the appropriate equilibrium concept is Nash equilibrium (that is, a profile of bids that is unilaterally stable).  There are many variants of Nash equilibrium (pure, mixed, correlated, etc.).  Our results will on the set of \emph{coarse correlated equilibria}.
%We quantify the price of anarchy with respect to Nash equilibria (i.e., bid profiles that are unilaterally stable) and with respect to
%the limit empirical distributions of no-regret repeated game-playing.
%It is well-known that such learning outcomes coincide with the solution concept of {\em coarse correlated equilibrium}, which is a superset of the set of mixed Nash equilibria and correlated equilibria.
%A joint distribution of bids $B$ constitutes a \textit{coarse correlated equilibrium} (CCE) if
%for every player $i$ and for any bid $b_i'$,
%\begin{equation}
%\textstyle{\E_{\rbid\sim B}[u_i(\rbid;\val_i)]\geq \E_{\rbid\sim B}[u_i(\rbid_i',\rbid_{-i};\val_i)].}
%\end{equation}
%The \emph{correlated price of anarchy} is defined as
%\begin{equation}
%POA = \max_{B \colon B \text{~is~} CCE} \frac{\opt(\vals)}{\E_{\rbid\sim B}[SW(X(\rbid))]}.
%\end{equation}

In the incomplete information setting we assume that each player's valuation $\val_i$ is drawn independently from
some commonly known distribution $\F_i$.  Let $\F=\F_1\times \ldots \times \F_n$ be the joint distribution.
A player's strategy is then a mapping $s_i(\val_i)$ from a valuation to a (potentially random) bid.
%
The prevailing solution concept under incomplete information is that of {\em Bayes-Nash equilibrium} (BNE).
A profile of strategies $s=(s_1,\ldots,s_n)$ is a BNE if, for every player $i$ and any valuation $\val_i$ in the support of $\F_i$, applying strategy $s_i(\val_i)$ maximizes the utility of player $i$ in expectation over the valuations and strategies of the other players.
%That is, for all $i\in[n]$, valuation $\val_i$, and bid $b_i' \in \Reals$,
%\begin{equation}
%\E_{\vals_{-i}\sim \F_{-i}}\E_{\rbid\sim s(\vals)}[u_i(\rbid;\val_i)]\geq \E_{\vals_{-i}\sim \F_{-i}}\E_{\rbid_{-i}\sim s_{-i}(\vals_{-i})}[u_i(\rbid_i',\rbid_{-i};\val_i)]
%\end{equation}
%
The inefficiency in the incomplete information setting is quantified using the \emph{Bayesian price of anarchy} (BPOA), which is defined similarly to the correlated price of anarchy above; the difference is that the welfare (both of the BNE and of the optimal outcome) is taken in expectation over the distribution of values.
%; i.e.,
%\begin{equation}
%BPOA = \max_{s \colon s \text{~is~} BNE} \frac{\E_{\vals\sim \F}[\opt(\vals)]}{\E_{\vals\sim \F,\rbid\sim s(\vals)}[SW(X(\rbid);\vals)]}.
%\end{equation}
%In other words, the price of anarchy for some equilibrium concept is at most $\rho$ if, at every equilibrium of the given class, the (expected) social welfare of the resulting allocation is at least $1/\rho$ of the optimal social welfare.

\paragraph{Efficiency of Simultaneous Single-Item Auctions}
%As discussed in the introduction, 
Recall that the price of anarchy for simultaneous item auctions can be unbounded when agents have arbitrary valuations \cite{Hassidim2011}. These bad examples hinge on the presence of an agent who has value only for a very large subset of items acquired together.  The inherent difficulty for such an agent is that 
%it is inherently difficult to bid safely on individual items; after all, 
if he wins only some, but not all, of his desired items, then he will still have to pay for his (worthless) winnings.  This leads to unnatural and inefficient bidding behavior at equilibrium.  The restriction to $\MOPH$-$k$ valuations deals with precisely this problem. An agent with a $\MOPH$-$k$ valuation obtains value from combinations of at most $k$ items, and hence the risk of winning only part of a combination is reduced.
% are interested in sets of up to $k$ items, and this is representable guaranteed to value subsets of items of size $k$ (if they in fact value anything at all).  
We are able to leverage this property for our price of anarchy bounds.

\iffalse
We the general framework for proving price of anarchy bounds: fix an equilibrium.  Choose potential deviations for each agent in which the agent tries to win his bundle in an optimal allocation.  Note that the total utility of these deviations is related to the optimal welfare (since each agent tries to win his optimal bundle) and is further bounded by the welfare of the equilibrium (by the equilibrium constraints).  Applying this framework requires ingenuity in selecting appropriate deviations.
\fi

%As in many prior analyses of simultaneous item auctions \cite{Feldman2013,Bhawalkar2011,Christodoulou2008,Hassidim2011,Syrgkanis2012}, the main step in our proof is to develop a good bidding strategy for an agent who wishes to win a set $S$ and faces a distribution over item prices.  Such a strategy precludes very inefficient equilibria, since an agent who obtains low welfare at equilibrium could apply the strategy to win his allocation in the optimal solution.  Our first key observation is that, due to the definition of $\MOPH$-$k$ valuations, an agent will have high value for winning a set $S$ so long as he wins each subset of $S$ of size at most $k$ with sufficiently high probability.  So then, how should an agent bid on a set $S$, given a distribution over item prices, such that he wins each subset of $S$ of size $k$ with sufficiently high probability?

%\blcomment{I rewrote the next few paragraphs to capture more of the argument, since we removed the PoA proof.  Not entirely sure how easily it can be understood by a non-expert.  Are there any unclear sections that should be cut / reworked?}
%\nicomment{I like it!}

Our price of anarchy analysis uses the following approach, employed by prior work on simultaneous item auctions \cite{Feldman2013,Bhawalkar2011,Christodoulou2008,Hassidim2011,Syrgkanis2012}. Consider a bidder $i$ who wishes to bid on a set $S$, given the opponents' strategies (which define a distribution over item prices, i.e.\ others' winning bids). We will develop a bidding strategy that guarantees high expected utility, unless the expected sum of prices is large relative to $v_i(S)$.
%
%the main step in our proof is to develop a good bidding strategy for an agent who wishes to win a set $S$ and faces a distribution over item prices.  
Such a strategy precludes very inefficient equilibria. Indeed, any agent who obtains low welfare at equilibrium could have applied our proposed strategy on his set in the optimal allocation. By the equilibrium condition, this deviation cannot improve his utility. Others must therefore be bidding highly on (and hence extracting high welfare from) his set in the optimal allocation. We can therefore charge this agent's optimal welfare against the high welfare of these other agents. Applying this argument to all bidders simultaneously implies that the welfare at equilibrium cannot be too low. Our goal, then, is to develop this supposed bidding strategy.

Our first key observation is that, due to the definition of $\MOPH$-$k$ valuations, we can focus on winning subsets of size $k$.  Indeed, suppose that agent $i$'s strategy guarantees that, for every subset $T$ of $S$ with $|T| = k$, the probability that $i$ wins every item in $T$ is at least $p$.  Then the expected value of his winnings is at least $p \cdot v_i(S)$, since he wins each hyperedge defining the value of $S$ with probability at least $p$. 
%So then, how should an agent bid on a set $S$, given a distribution over item prices, such that he wins each subset of $S$ of size $k$ with reasonable probability?

%that expected value for his winnings is (at least) linear in the probability that he wins any given subset of size $k$.  That is, if agent $i$ bids in such a way that, for every subset $T$ of $S$ with $|T| = k$, is won with probability at least $p$, then his expected value for his winnings will be at least $p \cdot v_i(S)$. , So then, how should an agent bid on a set $S$, given a distribution over item prices, such that he wins each subset of $S$ of size $k$ with sufficiently high probability?

Our second key idea extends an idea from \cite{Feldman2013}, namely that one ought to use the price distribution in defining the bidding strategy.  In \cite{Feldman2013}, the proposed bidding strategy was to draw a sample from the price distribution and then bid according to that sample.  This guarantees that each item is won with constant probability, and in the absence of complements this translates into a constant fraction of the value from set $S$.  However, in our case this is not sufficient:  the agent might obtain value only if he wins every item in certain subsets of size $k$.  Drawing a sample from the price distribution does not provide a sufficiently strong guarantee.  Rather, for each item in $S$, we draw $2k$ prices from the distribution of prices for that item, and then bid the maximum of these prices.  This guarantees that each item is won with probability at least $1 - 1/(2k+1)$, since the item is lost only if its true price is greater than all of the randomly selected prices.  A union bound then yields that any subset of $k$ items of $S$ is won with probability at least $1/2$. 
%Since the agent's value is generated from subsets of size at most $k$ (by the definition of MOPH-$k$ valuations), t
This implies that this bidding strategy gives the agent an allocation of high value (at least $v_i(S)/2$).  This translates into a strategy that yields good utility for the agent, unless the prices are relatively high in expectation (i.e., sum to at least $v_i(S)/2k$).  Applying this strategy to the argument above yields a PoA bound of $O(k)$.  We defer further details to Appendix \ref{sec:smoothness}.

%\bldelete{
%\nicomment{the following sounds weak, reword?}
%\vsedit{Thus the novelty that enables our main result is two-fold: first, an appropriate definition of restricted complementarities that allows for the expression of a large number of existing valuation classes, with both substitutes and complements, and second, the use of the order statistics of the prices when defining the deviation, together with a crucial use of the union bound so as to lower bound winning probabilities, when analysing the deviating utility of the player. Our formulation of the problem allows us to handle classes of hypergraph valuations with positive edges and negative hyperedges, by showing that first they can be expressed as a maximum over positive graphical valuations and then applying our proof for MOPH valuations. If we were
%to directly prove price of anarchy for such valuations we would have to argue as to why a player doesn't win negative hyperedges with too high
%probability. Proving both upper and lower bounds on the probability of winning is almost infeasible, when arguing about arbitrary price distributions.
%Thus our approach alleviates such difficulties, by distilling substitutabilities in a way that does not require arguing about winning probability upper bounds, but still allowing for the expression of some classes of negative hyperedge valuations.}
%}

%
\iffalse
\mfedit{In addition, by performing such a deviation the player pays at most $2k$ times the expected total price of the items in $S$. Thus, equilibrium conditions would then imply that either the player's utility in equilibrium is at least $1/2$ of his value of the set $S$, in which case he obtains an approximately equally well-valued set, or the expected revenue from that set $S$ is at least a $O(k)$ fraction of his value, in which case this value in aggregate is obtained by other players.} ... \textbf{Brendan: I gave up at this point.}
\fi
%
\ricomment{omitting. It seems a copy&paste of the result from Summary of Results section.}
\Omit{
\begin{theorem}\label{thm:non-smooth-poa}
For simultaneous first price auctions when bidders have $\MOPH$-$k$ valuations, both the correlated price of anarchy and the Bayes-Nash price of anarchy are at most $2k$.
\end{theorem}
}
%Theorem \ref{thm:non-smooth-poa} actually follows as a corollary of Theorem \ref{thm:smooth-poa}, described in Section \ref{sec:smoothness} in the Appendix. There we use the smooth mechanism framework \cite{Syrgkanis2013} and show a new "composability" theorem of smooth mechanisms for $\MOPH$-$k$ valuations, that degrades with $k$. The result then follows from known smoothness properties of a single-item first price auction.  

%However, to provide some intuition for our techniques, we provide a direct proof of a weaker version of Theorem \ref{thm:non-smooth-poa}.

\iffalse
\begin{theorem}\label{thm:mixed-poa}
For simultaneous first price auctions when bidders have $\MOPH$-$k$ valuations, the price of anarchy with respect to mixed Nash equilibria is at most $4k$.
\end{theorem}
\begin{proof}
%To simplify the proof, we will actually present a weaker bound of $4k$ on the price of anarchy, and present the proof only for mixed Nash equilibrium.
%The full proof of Theorem \ref{thm:non-smooth-poa} follows from the discussion following Theorem \ref{thm:smooth-poa}, later in this section.
%
Let $B\in \Delta(\R^{n\times m}_+)$ be a randomized bid profile that constitutes a mixed Nash equilibrium.  We will denote with $\rbid$ a random sample from distribution $B$.  A bid profile $\rbid$ defines an \emph{effective price} for each item $j$, given by $p_j = \max_i \rbid_{ij}$.  That is, the price of an item is the maximum bid placed on that item.  Distribution $B$ therefore induces a distribution over price profiles; let $P$ be this distribution of prices.  We will denote with $\rprice$ a random sample from $P$. Let $P_j$ be the marginal distribution of prices induced on item $j$.

We assume that each player's valuation over items is a $\MOPH$-$k$ valuation. Fix a player $i$, and let $v_i^*:2^M\to \nonnegR$ be the positive lower envelope of  $v_i$ of rank $k$, when the universe of items is restricted to $X_i^*$.  That is, $v_i(X_i^*) = v_i^{*}(X_i^*)$ and, for any set $T\subseteq [m]$, $v_i(T)\geq v_i^{*}(T)$.  We will denote with $w^*:2^M\to \nonnegR$ the positive hypergraph representation of $v_i^*$.
%Let $\Ell_i$ be the index set for the set of hypergraph-$k$ valuations used to express the valuation of player $i$.  Let $\ell_i^*\in \Ell_i$
%be the index of the hypergraph-$k$ valuation that matches player $i$'s value for his optimal set $X_i^*$, i.e. $v_i(X_i^*) = v_i^{\ell_i^*}(X_i^*)$ and, for any set $T\subseteq [m]$: $v_i(T)\geq v_i^{\ell_i^*}(T)$.

We will consider the following randomized strategy $B_i'$ for player $i$. For each item $j\in \opti$, select $2k$ samples from the distribution $P_j$ and set $B_{ij}'$ to the maximum of these samples,
%that follows the distribution of the maximum of $2k$ samples from the distribution $P_j$,
plus some negligible amount $\epsilon$ which goes to $0$. Denote with $\rbid_i'$ a random sample of $B_i'$.

%\geq \E\left[ \sum_{s\in \ESk{X_i(\rbid_i',\rbid_{-i})}}w_s^{*} - \sum_{j\in X_i(\rbid_i',\rbid_{-i})} \rbid_{ij}'\right]\\

Now consider the expected utility of player $i$ if he were to deviate to strategy $B_i'$.  This is
\begin{align*}
\E[u_i(\rbid_i',\rbid_{-i})]
=~& \E\left[ v_i(X_i(\rbid_i',\rbid_{-i}))  - \sum_{j\in X_i(\rbid_i',\rbid_{-i})} \rbid_{ij}'\right]
\geq \E\left[ v_i^*(X_i(\rbid_i',\rbid_{-i}))  - \sum_{j\in X_i(\rbid_i',\rbid_{-i})} \rbid_{ij}'\right]\\
\geq~& \E\left[ \sum_{S\subseteq X_i(\rbid_i',\rbid_{-i})}w^*(S) - \sum_{j\in X_i(\rbid_i',\rbid_{-i})} \rbid_{ij}'\right] 
\geq \sum_{S\subseteq \opti}w^*(S) \Pr\left[\wedge_{j\in S} (\rbid_{ij}'> \rprice_j)\right] - \sum_{j\in \opti} \E[\rbid_{ij}']
\end{align*}
where the last inequality follows from linearity of expectation.
%
Now observe that as $\epsilon$ goes to $0$, we have $\E[\rbid_{ij}'] \leq 2k\cdot\E_{\rprice_j \sim P_j}[\rprice_j]$ (since the expectation of the maximum of $2k$ samples is at most
the expectation of the sum).  Moreover, since $v_i^*$ has rank $k$, we have:
\begin{align*}
\E[u_i(\rbid_i',\rbid_{-i})]
& \geq \sum_{S\subseteq \opti: |S|\leq k}w^*(S)\Pr\left[\wedge_{j\in S} (\rbid_{ij}'> \rprice_j)\right] - \sum_{j\in \opti} \E[\rbid_{ij}']
\end{align*}
%
%
%
%Using these
%two properties, the expected utility of a player who deviates as described above can be lower bounded as follows:
%\begin{align*}
%\E[u_i(\rbid_i',\rbid_{-i})]=~& \E\left[ v_i(X_i(\rbid_i',\rbid_{-i}))  - \sum_{j\in X_i(\rbid_i',\rbid_{-i})} \rbid_{ij}'\right]
%\geq \E\left[ \sum_{s\in \ESk{X_i(\rbid_i',\rbid_{-i})}}w_s^{\ell_i^*} - \sum_{j\in X_i(\rbid_i',\rbid_{-i})} \rbid_{ij}'\right]\\
%\geq~&\sum_{s\in \ESk{\opti}}w_s^{\ell_i^*} \Pr\left[\forall j\in s: \rbid_{ij}'> \rprice_j\right] - \sum_{j\in \opti} \E[\rbid_{ij}']\\
%\geq~&\sum_{s\in \ESk{\opti}}w_s^{\ell_i^*} \Pr\left[\forall j\in s: \rbid_{ij}'> \rprice_j\right] - 2 k\cdot \sum_{j\in \opti} \E[\rprice_{ij}']
%\end{align*}
%
Moreover, the union bound implies that the probability of winning a set $S$ of items satisfies
\[ \Pr\left[\wedge_{j\in S}(\rbid_{ij}'> \rprice_j)\right]=1-\Pr\left[\vee_{j\in S}(\rbid_{ij}'\leq \rprice_j)\right] \geq 1-\sum_{j\in S}\Pr\left[\rbid_{ij}'\leq \rprice_j\right].\]
Since $\Pr[\rbid_{ij}' \leq \rprice_j]\leq \frac{1}{2k+1}$ (since this occurs only if $\rprice_j \sim P_j$ is larger than the $2k$ other independent draws from distribution $P_j$ that define $\rbid_{ij}'$), we get
\begin{align*}
\E[u_i(\rbid_i',\rbid_{-i})]\geq~&  \sum_{S\subseteq \opti: |S|\leq k}w^*(S)\cdot\left(1-\frac{k}{2k+1}\right)- 2k\cdot \sum_{j\in \opti} \E[\rprice_j]\geq~ \frac{1}{2} v_i(\opti)- 2k \cdot\sum_{j\in \opti} \E[\rprice_j].
\end{align*}
By invoking the equilibrium condition for player $i$ and then taking a sum over all players, we obtain
\begin{align*}
\sum_i \E[u_i(\rbid)]\geq \sum_i \E[u_i(\rbid_i',\rbid_{-i})]\geq \frac{1}{2}\sum_i v_i(\opti)-2k\cdot \sum_{j\in M}\E[\rprice_j]
\end{align*}
which implies that $\E[SW(X(\rbid))]+(2k-1)\E[\sum_{j\in[m]}\rprice_j]\geq \frac{1}{2}\opt$. Using the fact that expected revenue is at most the expected social welfare yields the desired bound.
\end{proof}
\fi

\paragraph{Second-Price Auctions and No-overbidding.} Our smoothness analysis in Appendix \ref{sec:smoothness} also applies  to the case of simultaneous second-price auctions, given that we restrict our attention to equilibria that satisfy the weak no-overbidding assumption (see Appendix \ref{sec:smoothness} for a definition).  Our surprising result is that the correlated and Bayes-Nash PoA are $2$ for arbitrary monotone valuations, given the weak no-overbidding assumption.  In other words, our PoA bounds for $\MOPH$-$k$ valuations do not degrade with $k$.
%\bldelete{Weak smoothness of a mechanism is essentially the same property as smoothness, but with the bids of the players
%replacing the payments on the right hand side and weak $(\lambda,\mu)$-smoothness implies a bound of $\lambda/(1+\mu)$ on
%the price of anarchy of every equilibrium that satisfies the weak no-overbidding assumption, i.e. no player is bidding in expectation more than than the expected value that he gets.}
%Thus subject to no-overbidding, simultaneous second-price auctions have correlated and Bayes-Nash price of anarchy of $2$ for arbitrary monotone valuations.
%%Such a property was known only for pure Nash equilibria by Fu et al. \cite{Fu2012}
%%and our smoothness argument extends it to
While this result seems quite positive, %However,
we suggest that it can be interpreted as indicating the strength of the no-overbidding refinement, especially in the presence of complementarities.
%Under high
%complementarities it is most probably true that
Indeed, the efficiency result is conditional on equilibrium existence, and the set of no-overbidding equilibria might be empty.
%%This is in contrast to our bound for simultaneous first price auctions.
%\mfcomment{We need to discuss either here or earlier in the paper existence for simultaneous first price auctions, or at least point to the appropriate literature --- I ended up adding a sentence in the end of the "our results" section.}


\paragraph{Composition of General Mechanisms.} As we show in Appendix \ref{SEC:COMPOSITION}, our analysis can be extended beyond simultaneous single-item auctions to the simultaneous composition of more general mechanisms, such as position auctions.  This shows that the results of \cite{Syrgkanis2013}, on the composability of smooth mechanisms,
extends to valuations that are $\MOPH$-$k$ across mechanisms.  We show that the PoA of the global mechanism, relative to the individual mechanisms, degrades linearly in the size of the complements.

}

==> poly-representation-leftovers.tex <==
% !TEX root=complements.tex

\begin{prop} \label{p:polyRepresentationMPH}
Given an $\MOPH$-$k$ set function with a representation that has at most polynomially many positive hypergraphs, each with at most polynomially many hyperedges, one can answer demand queries in polynomial time, using value queries.
\end{prop}

\begin{proof} %[of Proposition~\ref{p:polyRepresentationMPH}]
As observed in \cite{Abraham2012}, answering a demand query on one hypergraph is a supermodular maximization task, or equivalently, submodular minimization. Hence by known results, it can done in polynomial time, using value queries.
For polynomially many hypergraphs, compute an answer for each hypergraph separately, and return the best answer.
\end{proof}

\begin{prop}
Every $\MOPH$ representation (regardless of rank) of the submodular function $f(S) = \min[|S|,n/2]$ (which is in $\MOPH$-$1$) requires exponentially many hypergraphs.
\end{prop}

\begin{proof}
Consider two different sets $S$ and $T$ with $|S| = |T| = n/2$. Let $h$ be an arbitrary supermodular function (hence any positive hypergraph qualifies here) satisfying $h(Q) \le f(Q)$ for every set $Q$. We claim that either $h(S) \not= f(S)$ or $h(T) \not= f(T)$. This proves that at least ${n \choose n/2}$ hypergraphs are needed.

To prove the claim observe that $f(S \cap T) < n/2$ and $f(S \cup T) = n/2$. Suppose for the sake of contradiction that $h(S) = h(T) = n/2$. Then by supermodularity  $h(S \cap T) + h(S \cup T) \ge n$, implying that either $h(S \cap T) > f(S \cap T)$ or $h(S \cup T) > f(S \cup T)$. A contradiction.
\end{proof} 

==> positive-and-negative.tex <==
% !TEX root=complements.tex
In this section we focus on the parts from Theorem~\ref{t:expressiveness} that relate hypergraph valuations with rank $r$ and $\MOPH$-$r$ valuations.
In addition, we present preliminary results that advance our understanding toward a resolution of Conjecture~\ref{conj:quadratic}.

\paragraph{Graphical valuations}
%It is asserted in Theorem~\ref{t:expressiveness} that every graphical valuation is in $\MOPH$-2.
%In fact, 
We show that every hypergraph valuation that has positive rank~2 and arbitrary negative rank belongs to $\MOPH$-$2$. Recalling the example depicted in Figure~\ref{fig:hypergraph}, the hypergraph valuation on the left can indeed be expressed as the maximum over the $\PH$-$2$ valuations on the right. Our proof introduces a technique to charge negative hyperedges to positive edges, and is reduced to flow arguments on an appropriately defined graph.
The proof is deferred to Section~\ref{sec:neg-hyperedge-proof}.

\begin{theorem}\label{thm:hypergraph-vs-MOPH}
Every monotone set function with positive rank~2 and arbitrary negative rank is $\MOPH$-$2$.
\end{theorem}

%\mfcomment{We may want to push this proof forward to be in a section before the appendix. Currently it is in the appendix. To be discussed.}
We also show that every graphical valuation can be expressed as the sum of a $\PH$-$2$ function and a submodular function.
This proof appears in Appendix~\ref{app:decomposition}.
%\mfcomment{Do we have any applications of the above statement? and if not, is it significant?}



\paragraph{Symmetric functions}

%\blcomment{I'd recommend stating the more general result (that every monotone symmetric set function of rank $r$ is $\MOPH$-$R$ for $R \le 3r^2$) earlier in this paragraph.  From there, we could note that we think the true answer is tighter, and that we can verify the tight bounds for hypergraph ranks 3 and 4.}
%\mfcomment{I restructured this section as Brendan suggested. I indeed like it better.}

A set function $f$ is symmetric if $f(S) = f(T)$ whenever $|S| = |T|$.
Recall our conjecture (Conjecture~\ref{conj:quadratic}) that every hypergraph function with rank $r$ (positive or negative) is in $\MOPH$-$O(r^2)$.
While we were not able to establish this result for general hypergraph functions, the following theorem establishes that the assertion of the conjecture holds in the special case of symmetric functions.

\begin{theorem} \label{t:PleForAnyMonotoneSymmetricFunction} \label{thm:symmetricupperbound}
Every monotone symmetric set function of rank $r$ (positive and negative) is in $\MOPH$-$3r^2$.
\end{theorem}

%\ricomment{Changed a bit. I didn't feel comfortable with saying this was required. It seems so currently to us, but we cannot say we know for sure there is no trivial proof...}
The proof of Theorem~\ref{thm:symmetricupperbound} uses properties of the derivatives of polynomials of bounded degree (see \cite{Markov}). The proof is deferred to Section~\ref{sec:symmetric-upper}.
We actually conjecture a tighter bound of $\left\lceil \frac{r}{2} \right\rceil \left\lceil \frac{r+1}{2} \right\rceil$, and verify it for small ranks.
In particular, we show that every symmetric hypergraph function with rank $3$ is in $\MOPH$-$4$, and this is tight (i.e., there exists an hypergraph function with rank $3$ that cannot be represented by any $\MOPH$-$3$ function).
Similarly, we show that every symmetric hypergraph function with rank $4$ is in $\MOPH$-$6$, and this is tight.
For the upper bounds, we use our characterization of positive lower envelopes of symmetric functions (see Corollary~\ref{c:SymmetricPleClassificationByN-1}) and introduce an LP that characterizes a function that is the worst possible, accordingly. Then, by duality theorem, we bound the feasible solutions of this LP and conclude the theorem.
%The upper bounds use a non-trivial LP formulation of the problem, and
For the lower bounds we construct examples that are shown to satisfy the required properties
(see Appendix~\ref{app:smallRanks} for detailed proofs of both upper and lower bounds).
For other small values of $r$, we used computer-assisted simulations to compute the parameter $r$ of the $\MOPH$ hierarchy that is needed for each hypergraph rank. These simulations seem to support the precise formula we conjecture.


\paragraph{Hypergraph functions with positive rank $r$ and laminar negative hyperedges with arbitrary rank}

Using similar charging arguments to the ones used in the proof of Theorem~\ref{thm:hypergraph-vs-MOPH}, one can show that any hypergraph function with positive rank $r$ and arbitrary negative rank is in $\MOPH$-$r$, if every positive hyperedge that intersects a negative hyperedge is strictly contained in the negative hyperedge.
Additionally, Theorem~\ref{thm:expressiveness} asserts that every monotone function with positive rank $r$ and arbitrary negative rank is in $\MOPH$-$r$ if its negative hyperedges are laminar.
%TODO: compare with ABDR. consider writing this result also in the abstract or at least in the introduction.
The proof is deferred to Section~\ref{sec:laminar-proof}.


==> preliminaries-old.tex <==
% !TEX root = complements.tex

\paragraph{Combinatorial Auctions.} We consider the standard combinatorial auction setting, where $m$ items are to be sold to $n$ bidders. Each bidder $i$ has a valuation $v_i:2^{[m]}\rightarrow \R_+$ that assigns value to each set of items $S\subseteq [m]$.  
%We denote by $\V_i$ the set of possible valuations of player $i$. 
Throughout the paper we will assume that the valuations $v_i$ are monotone, i.e., for any $S\subseteq T: v_i(S)\leq v_i(T)$.
%We will denote by $\X\subseteq 2^{[m]\times n}$ the set of feasible allocations of items to bidders, i.e., such that no item is allocated to more than one bidder. 
A mechanism in a combinatorial auction setting defines some action space $\A_i$ for each of the bidders and we write $\A=\A_1\times \ldots \times \A_n$. Given an action profile $a \in \A$ the mechanism computes an outcome, which consists of
a feasible allocation vector $X(a)=(X_1(a),\ldots,X_n(a))$, where $X_i(a)\subseteq[m]$ is the set of items allocated to player $i$, and a payment vector $P(a)=(P_1(a),\ldots,P_n(a)) \in \R_+^n$.
We assume that players have quasi-linear utilities, i.e., the utility of player $i$ when the players play action profile $a$ is
%\begin{equation}
$u_i(a;v_i) = v_i(X_i(a))-P_i(a)$.
%\end{equation}

The social welfare or efficiency of any allocation is the total utility of all the bidders, plus the revenue of the auctioneer.  This is equal to the total value of the allocation: for any allocation $X$ and valuation profile $v=(v_1,\ldots,v_n)$, $SW(X;v)=\sum_{i\in [n]}v_i(X_i)$. Given a profile of valuations $v$ we will denote by $X^*(v)=(X_1^*(v),\ldots,X_n^*(v))$ the allocation that maximizes the social welfare; let $\opt(v)$ denote this optimal social welfare. When the valuation profile is fixed (i.e., not a variable),
such as in the complete information setting, we will often drop the dependence on $v$ in our notation.
% (e.g.,$u_i(a), SW(X),X_i^*,\opt$, etc.).
%
%\nicomment{It would be nice to eliminate unnecessary notation: $\X, \V, \A$ are essentially unused in other sections.}
%\vscomment{I elimitated $\X$ nd $\V$. I think $\A$ is useful to distinguish general mechanisms and general single item acutions 
%that have auctions to subsequently first price that have bids.}

\paragraph{Simultaneous Single-Item Auctions.} In this paper we analyse the following simple auction process: each of the $m$ items is sold using
a separate single-item auction. Formally, each bidder $i$ simultaneously submits a bid $b_{ij}$ for each item $j$. Write $b_i=(b_{i1},\ldots,b_{im})$
for the bid vector of player $i$.  Each item $j$ is then allocated
to the bidder who placed the highest bid on $j$ (breaking ties arbitrarily), and this winning bidder must pay his bid.  A player's utility under some bid profile $b=(b_1,\ldots,b_n)$ is then
%\begin{equation}
$u_i(b;v_i)  = v_i(X_i(b))-\sum_{j\in X_i(b)}b_{ij}.$
%\end{equation}
We will assume that each player has the option to bid zero and drop out of the auction, resulting in a utility of $0$. 
We will also give some results for the case where each item is sold via a second-price auction and under
which a player is asked to pay the second highest bid for each item he won.
%and hence each player's expected utility at any reasonable equilibrium concept will be non-negative.

\paragraph{Solution Concepts and Price of Anarchy.} We will analyze our auctions both in the complete and the incomplete information setting.
In the complete information setting it is assumed that the players have a fixed valuation profile $v$ that is common knowledge. The simultaneous auction process is then a normal form game of complete information. We will be interested in analysing the efficiency of Nash equilibria of this game (i.e., bid profiles that are unilaterally stable).  We are also interested in quantifying the efficiency of outcomes that result as limit empirical distributions of no-regret repeated game-playing. It is well-known that such learning outcomes coincide with the solution concept of the coarse correlated equilibrium, which is a superset of the set of mixed Nash equilibria
and correlated equilibria. A joint distribution of actions $A \in\Delta(\A)$ constitutes a \textit{coarse correlated equilibrium} (CCE) if 
for every player $i$ and for any action $a_i'\in \A_i$,
\begin{equation}
\textstyle{\E_{a\sim A}[u_i(a;v_i)]\geq \E_{a\sim A}[u_i(a_i',a_{-i};v_i)].}
\end{equation}
%That is, 
%no player can improve his utility by deviating unilaterally to a single action profile $a_i'$, given that the other players play according to action distribution $A$.

In the incomplete information setting we assume that each player's valuation $v_i$ is drawn independently from
some commonly known distribution $\F_i$.  Let $\F=\F_1\times \ldots \times \F_n$ be the joint distribution.
In an incomplete information  setting a player's strategy is not an action, but rather a mapping $s_i(v_i)$ from a valuation to a (potentially randomized) action.
%
In the incomplete information setting the prevailing solution concept is that of Bayes-Nash equilibrium. A profile of strategies $s=(s_1,\ldots,s_n)$ is a \emph{Bayes-Nash equilibrium} (BNE) if, for every player $i$ and any valuation $v_i$ in the support of $\F_i$, applying strategy $s_i(v_i)$ maximizes the utility of player $i$ in expectation over the valuations of the rest of the players. 
%\vsdelete{That is, for all $i\in[n]$, valuation $v_i$, and action $a_i'\in \A_i$,
%\begin{equation}
%\E_{v_{-i}\sim \F_{-i}}\E_{a\sim s(v)}[u_i(a;v_i)]\geq \E_{v_{-i}\sim \F_{-i}}\E_{a_{-i}\sim s_{-i}(v_{-i})}[u_i(a_i',a_{-i};v_i)]
%\end{equation}}

In the complete information setting we quantify inefficiency via the \emph{correlated price of anarchy}: %which is
\begin{equation}
\max_{a \colon a \text{~is~} CCE} \frac{\opt(v)}{SW(X(a))}.
\end{equation}
In the incomplete information setting we will quantify inefficiency with respect to the \emph{Bayes-Nash price of anarchy}, which is the same ratio but now both the equilibrium and optimal social welfare are taken in expectation over the distribution of values (e.g. $\E_{v\sim \F}[\opt(v)]$).
%\begin{equation}
%\max_{s \colon s \text{~is~} BNE} \frac{\E_{v\sim \F}[\opt(v)]}{\E_{v\sim \F,a\sim s(v)}[SW(X(a);v)]}
%\end{equation}
In other words, the price of anarchy for some equilibrium concept is at most $\rho$ if, at every equilibrium of the given class, the (expected) social welfare of the resulting allocation is at least $1/\rho$ of the optimal social welfare.

%\nicomment{ NSI: not sure we need to define all these notions for the conference version, can just use one (say NE which we don't even define here), and then remark that it extends to all these others.}
%\vscomment{At least I eliminated one of the two expressions.}






==> related-old.tex <==
%\blcomment{In general, the related work section seems very long, and seems to repeat some of what was stated in the description of our results.  Is there slack to cut it down?}

\paragraph{Expressiveness}

Our motivation for introducing the $\MOPH$ hierarchy comes from the study of combinatorial auctions. However, we remark that some classes of set functions received much attention in combinatorial optimization even prior to the interest in combinatorial auctions. This is especially true for the class of {\em submodular} functions on which there is a vast body of literature. We further remark that outside the context of combinatorial auctions, set functions are often not required to be monotone, and hence questions such as submodular function minimization (which can be solved in polynomial time, see~\cite{Cunningham}, for example) and maximization (which can be approximated within a factor of~$1/2$, see~\cite{BFNS}) are natural in these contexts. Similar questions may be relevant to our $\PLE$ hierarchy, which is a variation on the $\MOPH$ hierarchy that does not require monotonicity.

Following the interest in combinatorial auctions and the observation that the maximum welfare allocation problem is $\NP$-hard to approximate even with very poor ratio (see for example~\cite{LCS99} for the case of {\em single minded bidders} -- bidders that want one particular bundle of items), there has been extensive work on classification of monotone set functions. We distinguish between two types of classifications. One is that of {\em restricted classes} of set functions, and the other is {\em inclusive hierarchies} that capture all monotone set functions.

{\bf Restricted classes of monotone set functions.}
Lehmann, Lehmann and Nisan~\cite{Lehmann2001} initiated a systematic classification of set functions without complementarities. The main classes in their classification (in order of increasing expressiveness) are {\em linear} (a.k.a. {\em additive}), {\em gross substitutes} (a class introduced by Kelso and Crawford~\cite{KC82}), {\em submodular}, {\em $\XOS$} (the terminology for this class is taken from earlier work of Sandholm~\cite{Sandholm}), and {\em complement free} (a.k.a. {\em subadditive}). The maximum welfare in combinatorial auctions can be solved in polynomial time when the valuation functions of players are either in the class of linear functions or gross substitutes functions. Subsequent research showed that the maximum welfare can be approximated within a ratio somewhat better than $1 - 1/e$ in the submodular case~\cite{FV}, $1 - 1/e$ in the $\XOS$ case~\cite{DS2006} and~2 in the subadditive case~\cite{Feige2006}. These approximation algorithms assume {\em demand queries} access to the valuation functions, though for the submodular case, if one is satisfied with a $1 - 1/e$ ratio, then {\em value queries} suffice~\cite{Vondrak}.

It follows from the definitions that $\MOPH$-1, the first level of our hierarchy, coincides with the class of $\XOS$ functions.

Conitzer, Sandholm, and Santi~\cite{Conitzer2005}
%Acemoglu, Candogan, Ozdaglar, and Parrilo~\cite{Acemoglu2012} 
consider the class of monotone functions that have what they refer to as {\em graphical valuations}. Namely, every item has a value, and every pair of items (edge of the graph) has a value (positive if the items are complements, negative if they are substitutes, and~0 if they are independent), and the value of a set of items is the sum of values of items and edges within the set. It will follow (though this is a nontrivial claim that requires a proof) that the class of graphical valuations is contained in $\MOPH$-2, the second level of our hierarchy.

Abraham, Babaioff, Dughmi, and Roughgarden~\cite{Abraham2012} consider a hierarchy of valuation functions that allows only complements but no substitutes. In particular, submodular functions cannot be expressed in this hierarchy, and moreover, even some supermodular functions cannot be expressed in this hierarchy. The $k$-th level of this hierarchy, $\PH$-$k$, contains those functions that can be represented by a hypergraph in which edges have rank at most $k$, all vertices and hyperedges have non-negative values, and the value of a set of items is the sum of values of items and hyperedges within the set. In is shown in~\cite{Abraham2012} that the maximum welfare problem can be approximated within a ratio of~$k$ if all valuation functions are in $\PH$-$k$. They also discuss mechanisms that are truthful in expectation, but the approximation ratios achieved by their mechanisms deteriorate with the total number $m$ of items, even if $k$ remains fixed.

It follows from the definitions that for every $k$, $\PH$-$k$ is strictly contained in $\MOPH$-$k$.


{\bf Inclusive hierarchies of monotone set functions.} Feige and Izsak~\cite{Feige2013} introduced a hierarchy of monotone set functions, parameterized by the so-called {\em supermodular degree}. Unlike the $\MOPH$ hierarchy whose levels are numbered from~1 to~$m$, the levels of the supermodular degree hierarchy are numbered from~0 to $m-1$, and one should keep this in mind when comparing levels of these hierarchies. The functions with supermodular degree~0 are the submodular functions. As shown in~\cite{Feige2013}, there is a greedy algorithm that approximates the welfare maximization problem within a ratio of $k+2$ if the supermodular degree of all valuation functions is at most $k$.

It is not difficult to show that for every $k$, functions of supermodular degree $k$ are in $\MOPH$-$(k+1)$. For the other direction, there are functions in $\MOPH$-2 that cannot even be approximated by functions of low supermodular degree (e.g., functions of supermodular degree $\sqrt{m}$ approximate them only within a ratio of $\Omega(\sqrt{m})$).

Another inclusive hierarchy that one may consider is similar to the $\PH$ hierarchy mentioned above, but without the restriction that hyperedges have positive values. Namely, level $k$ of the {\em hypergraph} hierarchy contains all those monotone functions whose hypergraph representation includes hyperedges up to rank $k$. Level~1 of this hierarchy is the linear functions, level~2 coincides with the graphical valuations mentioned above, and level $m$ captures all monotone set functions (on $m$ variables). There are no known positive results that connect between approximation ratios of the maximum welfare problem and the level of the valuation functions in the hypergraph hierarchy.

We conjecture that every function in level $k$ of the hypergraph hierarchy is in $\MOPH$-$O(k^2)$. For $k=2$ we confirm this conjecture (and even prove stronger results), and for every $k$ we prove the conjecture in the special case of symmetric functions. For the other direction, there are functions in $\MOPH$-1 that are not contained in any fixed level (independent of $m$) of the hypergraph hierarchy, and moreover, they cannot even be approximated within a fixed level of the hypergraph hierarchy.

%A series of papers studies the efficiency of equilibria of simple combinatorial auctions that are based on running separate item auctions (simultaneously or sequentially) for each item, showing constant approximate efficiency \cite{Bikhchandani1999,Christodoulou2008,Bhawalkar2011,Hassidim2011,Feldman2013,PaesLeme2012,Syrgkanis2012a}.
%All of these works assume that players' valuations are complement-free.

The $\XOS$ class introduced in~\cite{Lehmann2001} is based on ``OR" and ``XOR" operations previously introduced in~\cite{Sandholm}, but with the restriction that ``OR" operations are applied on single items. Removing this restriction and allowing operations on bundles, one obtains an $\XOS$ hierarchy parameterized by the size of the largest bundle. (The $\XOS$ hierarchy was suggested to us in personal communication by Noam Nisan.) While $\XOS$-$k$ and $\MOPH$-$k$ coincide for $k=1$, $\MOPH$-$k$ is strictly better than $\XOS$-$k$. It can be shown that $\XOS$-$k$ is contained in $\MOPH$-$k$, whereas there are functions in $\MOPH$-2 that cannot even be approximated in $\XOS$-$k$ for any constant $k$. 
(The proof uses the $\PH$-2 function used in Section~\ref{app:incompatible}).

\paragraph{Welfare approximation}

%\blcomment{If we are putting the PoA related work here, then I think we we should also move the related algorithmic work here as well.  That is, the second half of the first paragraph in "Restricted Classes of Monotone Set Functions."}

The complement-free valuations introduced in \cite{Lehmann2001} have also been studied in the game-theoretic context of equilibria in simultaneous single-item auctions.  It has been established that the Bayes-Nash and Correlated price of anarchy of this auction format, with a first-price payment rule, are at most $e/(e-1)$ in the $\XOS$ case~\cite{Syrgkanis2012a} and at most~2 in the subadditive case~\cite{Feldman2013}. For the second-price payment rule, these bounds become 2 for $\XOS$~\cite{Christodoulou2008} and $4$ for subadditive~\cite{Feldman2013}. These results build upon a line of work studying non-truthful item auctions for complement-free valuations \cite{Bikhchandani1999,Bhawalkar2011,Christodoulou2008,Hassidim2011,PaesLeme2012}.

Equilibrium analysis of non-truthful auctions has been applied to several other settings such as position auctions \cite{Caragiannis2012}, bandwidth allocation mechanisms \cite{Syrgkanis2013}, combinatorial auctions with greedy allocation rules \cite{Lucier2010}, and multi-unit auctions \cite{Markakis2012}. Recently, Roughgarden \cite{Roughgarden2012}, Syrgkanis \cite{Syrgkanis2012} and Syrgkanis and Tardos \cite{Syrgkanis2013} proposed general smoothness frameworks for bounding the social welfare obtained in equilibria of (compositions of) mechanisms. 

==> results-old.tex <==

%We now provide a summary of our

We obtain results on the expressiveness power of the $\MOPH$-$k$ hierarchy and on the approximability of social welfare in combinatorial auctions with $\MOPH$-$k$ valuations, from both algorithmic and game-theoretic perspectives.
%
The first theorem establishes the expressiveness power of our hierarchy.

\begin{theorem} \label{t:expressiveness} \label{thm:expressiveness}
%The $\MOPH$ hierarchy captures many existing hierarchies, as follows:
The $\MOPH$ hierarchy captures the following existing classes, as follows:
\begin{enumerate}
\item The class $\MOPH$-$1$ is, by definition, equivalent to the class $\XOS$ (defined by Lehmann, Lehmann and Nisan \cite{Lehmann2001}).

\item Every monotone graphical valuation (defined by Conitzer et al. \cite{Conitzer2005}) is in $\MOPH$-2. Furthermore, every monotone function with positive rank~2 is $\MOPH$-2 (see Section~\ref{sec:positive-and-negative}).

%\ricomment{I'm not sure about the reference. Have they been the first ever to consider graphical valuations? I think it was studied years before. Wasn't it?}
%\ricomment{I'd consider adding here a furthermore clause for arbitrary negative edges.}
%\blcomment{Note also that ``positive rank'' hasn't yet been defined.}

\item Every function that has a positive hypergraph representation of rank $k$ (defined by Abraham et al. \cite{Abraham2012}, see Section~\ref{sec:prelims}) is, by definition, in $\MOPH$-$k$.
%Furthermore, every monotone function that has a hypergraph representation with {\em positive rank} $k$ and laminar %negative hyperedges (with arbitrary rank) is in $\MOPH$-$k$ (see Section~\ref{}).

\Omit{\item Every monotone function that has a hypergraph representation with positive rank $k$ and laminar negative hyperedges (with arbitrary rank) is in $\MOPH$-$k$ (See Section~\ref{}).}
%\ricomment{We haven't defined yet positive rank. Moreover, I don't think it is a well known notion. It is better to define it before this theorem, or at least to add a reference to preliminaries (better to define before, if flows).}
%\ricomment{We can consider adding here a comparison to ABDR (i.e. to $\PH$-$k$). Can also move this item to be a furthermore clause for $\PH$-$k$. This way we have one item less and we also emphasize we have strictly more than ABDR in the same item. In any case, I put it right after the $\PH$-$k$ item.}

%\blcomment{I'd actually propose not mentioning this item; it seems out of place since the other items are classes considered elsewhere.  Instead, we could pose our conjecture that hypergraph representations can be captured by our hierarchy, and state that we establish this for certain rich subclasses that we'll define later, with a forward pointer to the appropriate section.}

\item Every monotone function that has supermodular degree $k$ (defined by Feige and Izsak \cite{Feige2013}) is in $\MOPH$-$(k+1)$ (See Section~\ref{sec:supermodular}).
%%\item Every function that can be represented as XOR of ORs of bundles of size $k$ (as defined by Sandhold \cite{}) is in $\MOPH$-$k$ (See Section~\ref{}).

\end{enumerate}
\end{theorem}
%\ricomment{I think we should consider an alternative wording for the following 2 sentences (limitations seems problematic to me).}
%The introduction of a new hierarchy is desired, in part, due to the limitations of previous hierarchies.
%To demonstrate these limitations, we define the following notion of approximation:

We further establish that the converse direction does not hold, even in an approximate sense, and conclude that
the $\MOPH$-$k$ hierarchy is \emph{strictly} more expressive than many existing hierarchies.
Specifically, we show that $\MOPH$-$1$ and $\MOPH$-$2$ contain functions that cannot be \emph{approximated} by functions in low levels of other hierarchies.
Before stating the result, we define the notion of approximation.

\begin{defn} \label{def:approximate}
\label{def:approximation}
We say that a set function $f$ approximates a set function $g$ within a ratio of $\rho \ge 1$ if there are $\rho_1$ and $\rho_2$ such that for every set $S$
$\rho_1 \le \frac{f(S)}{g(S)} \le \rho_2$, and $\frac{\rho_2}{\rho_1} \le \rho$.
\end{defn}


%The following proposition shows that the previous hierarchies are mutually incomparable in the sense of the above definition.
%These results are discussed in Section~\ref{}).

%\blcomment{Rather than describe the issue as ``incompatibility'' in the statement of Proposition \ref{prop:incompatible}, could we instead state the proposition as establishing that $\MOPH$ is strictly more expressive than many existing hierarchies, even with respect to approximation?  This would make it clear that Proposition \ref{prop:incompatible} is about $\MOPH$, rather than being about the space of hierarchies more generally.}

We are now ready to state the proposition. Its proof is deferred to Appendix~\ref{app:incompatible}.

\begin{prop} \label{prop:incompatible}
There are functions in very low levels of the $\MOPH$ hierarchy that cannot be approximated well even at relatively high levels of other hierarchies, as follows:
\begin{enumerate}
\item There exists a submodular function (i.e., supermodular degree $0$, $\MOPH$-$1$) such that
\begin{enumerate}
\item A graphical function cannot approximate it within a ratio better than $\Omega(m)$.
\item A positive hypergraph function cannot approximate it within a ratio better than $m$.
\item A hypergraph function of rank $k$ (both negative and positive) cannot approximate it within a ratio better than $\Omega(\frac{m}{k^2})$, for every $k$.
\end{enumerate}
\item There exists a $\PH$-2 function (i.e., $\MOPH$-2) such that every function of supermodular degree $d$ cannot approximate it within a ratio better than $\Omega(m/d)$.
\end{enumerate}
\end{prop}

With the new hierarchy at hand, we are in a position to revisit fundamental algorithmic and game-theoretic problems about welfare maximization in combinatorial auctions.
Our results are reassuring: we obtain good approximation ratios for settings with valuations that lie in low levels of the $\MOPH$-$k$ hierarchy.
From the algorithmic perspective, we provide a polynomial time $(k+1)$-approximation algorithm for the welfare maximization problem when valuations are $\MOPH$-$k$ (assuming access to demand oracles).

%\ricomment{I added a label. Should be referenced also from the section. Perhaps also the same for the first theorem.}
\begin{theorem} \label{t:algorithmic}
If all agents have $\MOPH$-$k$ valuations, then there exists an algorithm that gives $k+1$ approximation to the optimal social welfare.
This algorithm runs in polynomial time given an access to demand oracles for the valuations.
\end{theorem}

Our approximation algorithm first solves the configuration linear program for welfare maximization introduced by \cite{DNS}.
As is well known, solving this LP can be done in polynomial time using demand queries.
We then round the solution to the LP so as to get an integer solution. Our rounding technique is oblivious and does not require access to demand queries.
By analyzing the integrality gap, it is established that our rounding technique is nearly best possible.

The second setting we consider is a simultaneous first-price auction --- where each of the $m$ items is sold via a separate single-item auction.
We quantify the welfare loss in this simple auction when bidders have $\MOPH$-$k$ valuations.
%\ricomment{If it's $2k$, I think it is better to just say it.}
We find that the price of anarchy is at most $2k$.

\begin{theorem} \label{t:poa}
For simultaneous first price auctions, when bidders have $\MOPH$-$k$ valuations, both the correlated price of anarchy and the Bayes-Nash price of anarchy are at most $2k$.
\end{theorem}

Our proof technique extends the analysis for complement-free valuations in \cite{Feldman2013} and the smoothness framework introduced in \cite{Syrgkanis2013} to settings with complementarities.

\paragraph{Extensions}
One of the main open problems suggested by this work is the relation between hypergraph valuations of rank $k$ and $\MOPH$-$k$ valuations.
We make the following conjecture:
\begin{conj} \label{conj:quadratic}
Every hypergraph function with rank $k$ (positive or negative) is in $\MOPH$-$O(k^2)$.
\end{conj}
We make partial progress toward the proof of this conjecture.
For $k=2$ this conjecture is confirmed in Theorem~\ref{thm:hypergraph-vs-MOPH}, whose proof is based on flow arguments.
For larger $k$, we show that any monotone function that has a hypergraph representation with positive rank $k$ and laminar negative hyperedges (with arbitrary rank) is in $\MOPH$-$k$ (See Section~\ref{sec:positive-and-negative}).

This conjecture is also confirmed for the special case of symmetric functions, for any $k$, using Markov inequalities on derivatives of polynomials (See Section~\ref{sec:positive-and-negative}).
For symmetric functions, we actually conjecture a more precise bound of $\left\lceil \frac{k}{2} \right\rceil \left\lceil \frac{k+1}{2} \right\rceil$, which is suggested by a computer-assisted simulation based on a non-trivial LP formulation.
%\ricomment{TODO (Rani): add here a few words about the technique.}
For the special cases of symmetric hypergraph functions of ranks $k=3$ and $k=4$, we show analytically that they are in $\MOPH$-4 and $\MOPH$-6, respectively, and that this is tight.  %\blcomment{TODO: say a few words about hypergraph valuations with laminar negative edges}

Most of our expressiveness results showing that a certain function belongs to $\MOPH$-$k$ are established by showing that the function satisfies a certain requirement that we refer to as the Positive Lower Envelope (PLE) condition.
We also observe that, together with monotonicity, this requirement becomes a sufficient and necessary condition for membership in $\MOPH$-$k$.
This observation motivates the definition of a new hierarchy, referred to as $\PLE$.  The class $\PLE$-$k$ contains $\MOPH$-$k$, but also includes non-monotone functions.
%but without the monotonicity requirement.
%\ricomment{Is it accurate?}
It should be noted that while monotonicity is a standard assumption in the context of combinatorial auctions, $\PLE$ can be applicable outside the scope of combinatorial auctions.
Moreover, our approximation results in Theorems~\ref{t:algorithmic} and~\ref{t:poa} carry over to $\PLE$-$k$ functions, assuming that goods are allowed to remain unallocated.
%Exploring the relations between the expressiveness of hypergraph valuations and the $\PLE$ hierarchy is a fertile ground for future research.
%Applying the $\PLE$ hierarchy to optimization problems involving non-monotone set functions is a fertile ground for future research.
See Section~\ref{sec:non-monotone} for further discussion.

[Place Holder for something about $\PLE$ hierarchy + reference to appendix]
[Place Holder for limitations + reference to proofs regarding it in an appendix]


==> smoothness.tex <==
% !TeX root = complements.tex

In this section we show that the simultaneous first price auction is actually a Smooth Mechanism as defined in \cite{Syrgkanis2013}. The latter property then 
directly implies that any efficiency guarantee extends to Bayes-Nash equilibria of the incomplete information setting as well as to no-regret learning outcomes. For completeness we first present the definition and the main implication of smooth mechanisms. 

\begin{defn}[\cite{Syrgkanis2013}]
A mechanism $M$ is $(\lambda,\mu)$-smooth if for any valuation profile $v$ there exists an action profile $a_i^*(v)$ such that for all $a\in \A$:
\begin{equation}
\sum_i u_i(a_i^*(v),a_{-i};v_i)\geq \lambda \opt(v) - \mu \sum_i P_i(a)
\end{equation}
\end{defn}

\begin{theorem}[\cite{Syrgkanis2013}] If a mechanism is $(\lambda,\mu)$-smooth then the Bayes-Nash and the correlated
price of anarchy is at most $\mu/\lambda$.
\end{theorem}

We will analyze a generic simultaneous single-item auction where each item $j$ is sold via an auction with allocation function $X^j:\A^j\rightarrow [n]$ and payment function $P^j:\A^j\rightarrow \R^n_+$, where $\A^j=\A_1^j\times\ldots \A_n^j$, is some 
action space defined by the auction. We will show that if each individual single-item auction is a $(\lambda,\mu)$-smooth mechanism
and bidders have MOH-$k$ valuations then the simultaneous signle-item auction
is $\left(1-k+\min\left\{\lambda,1\right\}\cdot k,\mu\right)$-smooth. Subsequently, we will invoke the smoothness of the first-price auction
known from the literature, to show our result for simultaneous first-price auctions. 

We will first show that if we prove smoothness of the simultaneous auction for hypergraph-$k$ valuations then this immediately
implies smoothness for MOH-$k$ valuations and then we will prove smoothness for the class of hypergraph-$k$ valuations. 
\begin{lemma}\label{lem:hypergraph-to-moh}
If a simultaneous single-item auction game is $(\lambda,\mu)$-smooth for hypergraph-$k$ valuations then it is also 
$(\lambda,\mu)$-smooth for the class of MOH-$k$ valuations.
\end{lemma}
\begin{proof}
Consider a valuation profile $v$.  Let $\ell_i^*$ be player $i$'s index of the hypergraph-$k$ valuation in $\Ell$ that matches his 
value for his optimal allocation $X_i^*(v)$ and denote with $v_i^*$ the actual valuation. Thus by definition: $v_i(X_i^*(v)) = v_i^*(X_i^*(v))$ and for any set $T\subseteq [m]$: $v_i(T)\geq  v_i^*(T)$.

Observe that a player's utility under valuation $v_i$ is at least as much as his utility under $v_i^*$: $u_i(a;v_i)\geq u_i(a;v_i^*)$. 
Now consider the smoothness deviations $a_i^*(v^*)$ that correspond to valuation profile $v^*=(v_1^*,\ldots,v_n^*)$, which exist by the assumption that the mechanism is smooth for hypergraph-$k$ valuations. Then we get that for any action profile:
\begin{align*}
\sum_i u_i(a_i^*(v^*),a_{-i};v_i)\geq~& \sum_i u_i(a_i^*(v^*),a_{-i};v_i^*)\geq \lambda\opt(v^*)-\mu\sum_i P_i(a)\\
\geq~& \lambda SW(X^*(v);v^*)-\mu \sum_i P_i(a) = \lambda \opt(v) - \mu \sum_i P_i(a)
\end{align*}
\end{proof}

\begin{theorem}\label{thm:smooth-poa}
The game defined by running $m$ simultaneous $(\lambda,\mu)$-smooth single-item auctions is $\left(1-k+\min\left\{\lambda,1\right\}\cdot k,\mu\right)$-smooth, when players have MOH-$k$ valuations.\end{theorem}

For the case when each single-item auction is a first price auction then we know by \cite{Syrgkanis2013} that each auction is $\beta\cdot(1-e^{-1/\beta}),\beta)$-smooth for any $\beta$.
Thus we get that for any $\beta$ the simultaneous first price auction with MOH-$k$ valuations is $(1-(1-\beta\cdot(1-e^{-1/\beta}))\cdot k,\beta)$-smooth, which gives the optimal 
bound of $\frac{1}{1-(k-1)\log(\frac{k}{k-1})}\leq k(2-e^{-k})$ on the price of anarchy for $\beta=\log(\frac{k}{k-1})$, which leads to the tight bound claimed in Theorem \ref{thm:non-smooth-poa}.


==> supermodular.tex <==
% !TEX root=complements.tex

We explore the relation between $\MOPH$-$k$ functions and the recently introduced notion of the supermodular degree of Feige and Izsak \cite{Feige2013}. For completeness we revisit their definitions. Given a set function $f:2^M \to \nonnegR$, the marginal value conditional on some set $S$, is a set function $f(\cdot | S): 2^M\to \nonnegR$ defined as:
\begin{equation}
f(T~|~S) = f(T\cup S)-f(S)
\end{equation}
For monotone submodular functions, $f(T~|~S)$ is non-increasing in $S$, i.e. it exhibits non-increasing marginals. The supermodular degree of a function, captures intuitively how many violations of this non-increasing marginal property can be associated with any given item in the ground set.

\begin{defn}[Supermodular Degree \cite{Feige2013}] Given a set function $f:2^M\to \nonnegR$, an item $j\in M$ is supermodularly dependent on an item $j'\in M$ if there exists a set $S\subset M$ under which they exhibit strictly increasing marginals:
$f(j~|~S+\{j'\}) > f(j~|~S)$.
The supermodularly dependent set of an item is the set of all its supermodularly dependent items. The supermodular degree of a function is the size of the largest supermodular dependent set among all items.\footnote{Observe that the supermodular dependency relation is symmetric, as it followed directly from $f(j~|~S+\{j'\})-f(j~|~S) = f(j'~|~S+\{j\})-f(j'~|~S)$.}
\end{defn}

The definition of the supermodular degree gives rise to the supermodular degree hierarchy:
\begin{defn}[Supermodular Degree-$k$ ($\SMD$-$k$) class]  A set function $f:2^M\to \nonnegR$ is in $\SMD$-$k$
if it has supermodular degree at most $k$.
\end{defn}

%\mfcomment{I omitted a discussion here that is subsumed by stronger results in Proposition 2.}
\Omit{For a PH-$k$ valuation the supermodularly dependent set of an item is the union of all the hyperedges with strictly positive weights that contain it. Thus, for a graphical valuation with positive weights the supermodular degree is the maximum degree of any node, which can be arbitrarily larger than $k$. In other words, there exist set functions that are in $\MOPH$-$2$ but are not in $\SMD$-$k$ for any $k\leq n-1$. \vsedit{In fact it can be shown that there are even functions in $\MOPH$-$1$, that have supermodular degree of $m-1$.}
}
%\mfcomment{We actually know more than that: that even $\MOPH$-$1$ might be $\SMD-(n-1)$}}

%Most importantly we show that the supermodular degree can only be an overestimate of the allowed complementarity of a set function when compared to the $\MOPH$-$k$ measure. Specifically, we show that a set function with supermodular degree $k$
%always admits a $\MOPH$-$(k+1)$ representations (the plus one is only due to notational inconsistency).
%%We defer the proof to the Appendix.
%\vscomment{Assuming we go with this formulation, I am thinking would be good to slightly alter the supermodular degree to avoid this notational consistency so that we get a theorem of the form $\SMD-k \subset \MOPH-k$.}
%\mfcomment{I like this idea.}

Theorem~\ref{t:expressiveness} asserts that every function in $\SMD$-$k$ is in $\MOPH$-$(k+1)$.
Intuitively, if a function is in $\SMD$-$k$, every single item depends positively on at most $k$ other items.  As it turns out, one can use this property to construct positive lower envelopes for such a function, which establishes that %, and therefore it is not surprising that 
the function belongs to $\MOPH$-$k$. %Yet, this type of connections requires subtle arguments, and requires a formal proof. 
The formal proof is deferred to Section~\ref{sec:supermodular-proof}.

%\nicomment{can we also say that mph-k+1 includes many more functions than smd-k?}
%\mfcomment{I moved the statement and proof to Section~\ref{sec:supermodular-proof}.}


==> symmetric-proof.tex <==
\begin{thm}
For every $r$, every normalized monotone symmetric set function of rank $r$ has a lower envelope of rank $R \le 3r^2$ that has a positive hypergraph representation.
\end{thm}

\begin{proof}
Let $f$ be a normalized monotone symmetric set function of rank $r$, and let $h$ be its hypergraph representation. Consider the following normalized monotone symmetric set function $g$ defined by its positive hypergraph representation $p$: $p(S) = f(U)/{n \choose R}$ if $|S| = R$, and $p(S) = 0$ otherwise. As all four functions $f,h,g,p$ are symmetric, we shall change notation and replace $f(S)$ by $f(|S|)$. As special cases of this notation, $f(U)$ is replaced by $f(n)$, and $f(\phi)$ is replaced by $f(0)$.

We claim that $g$ is a lower envelope for $f$. There are three conditions to check. Two of them trivially hold, namely, $g(0) = f(0) = 0$, and $g(n) = {n\choose R}p(R) = f(n)$. The remaining condition requires that $g(k) \le f(k)$ for every $1 \le k \le n-1$. This trivially holds for $k < R$ because in this case $g(k) = 0$, whereas $f(k) \ge 0$. Hence the main content of our proof is to establish the inequality $g(k) \le f(k)$ for every $R \le k \le n-1$.


Suppose for the sake of contradiction that there is some $f$ that serves as a negative example, namely, that for this $f$ there is $R \le k \le n-1$ for which $g(k) > f(k)$. Moreover, among all possible negative examples (of rank $r$), consider the one with the smallest value of $n$. We claim that in this case we may take $k = n-1$. Suppose otherwise, that $g(n-1) \le f(n-1)$ and for some other $k < n-1$ it holds that $g(k) > f(k)$. Then scale $g$ by multiplying it by $f(n-1)/g(n-1)$. For the new $g$ it holds that $g(n-1) = f(n-1)$ and $g(k) > f(k)$, serving as a negative example with smaller $n$.

Observe that $g(n-1) = {n-1 \choose R}f(n)/{n \choose R} = \frac{n-R}{n}f(n)$. We now develop some machinery in order to show that $f(n-1) \ge \frac{n-R}{n} f(n)$.


\begin{proposition}
\label{pro:polynomial}
There is some polynomial $F$ of degree at most $r$ such that $F(X) = f(x)$ whenever $x \in \{0,1, \ldots, n\}$.
\end{proposition}

\begin{proof}
The polynomial is $F(x) = \sum_{i=1}^r {x \choose i}h(i)$, where $h(i)$ are constants derived from the hypergraph representation of $h$, and $x \choose i$ is the polynomial $\frac{1}{i!}x(x-1) \ldots (x - i + 1)$.
\end{proof}

Given that $F(x)$ is a polynomial of degree at most $r$, we shall use Markov's inequality regarding derivatives of polynomials~\cite{markov}.

\begin{lemma}
\label{lem:markov}
Let $p$ be a polynomial of degree $d$ and let $p'$ denote its derivative. Then
$$\max_{-1 \le x \le 1} |p'(x)| \le d^2\max_{-1 \le x \le 1} |p(x)|$$
\end{lemma}

By a simple transformation of the range on which the polynomial is defined, Lemma~\ref{lem:markov} implies that for our polynomial $F(x)$ the following holds:

\begin{equation}\label{eq:markov}
\max_{0 \le x \le n} |F'(x)| \le \frac{2r^2}{n}\max_{0 \le x \le n} |F(x)|
\end{equation}

Let $M = \max_{0 \le x \le n} |F(x)|$ and let $0 \le y \le n$ be such that $|F(y)| = M$. If $y$ is an integer then monotonicity of $f$ (and hence of $F$ on integer points) implies that $M = f(n)$. However, $y$ need not be integer. In that case $i < y < i+1$ for some $0 \le i \le n-1$. Let $m = \max[|F(i)|,|F(i+1)|]$. Then

$$M \le m + \frac{1}{2}\max_{i \le x \le i+1}[|F'(x)|] \le f(n) + \frac{1}{2}\max_{0 \le x \le n}|F'(x)| \le f(n) + \frac{r^2}{n}M$$
where the last inequality was derived from inequality~(\ref{eq:markov}). As $n \ge R \ge 3r^2$ we obtain that $M \le 3f(n)/2$.

Now we use inequality~(\ref{eq:markov}) to bound $f(n-1) = F(n-1)$ from below.

$$F(n-1) \ge f(n) - \max_{0 \le x \le n}F'(x) \ge f(n) - \frac{2r^2}{n}M \ge f(n) - \frac{3r^2}{n}f(n)$$

Using $R \ge 3r^2$ we have that $f(n - 1) \ge (1 - \frac{R}{n})f(n) = g(n-1)$, as desired.
\end{proof}


==> welfare-max.tex <==
% !TEX root=complements.tex

\vscomment{I thought merging the two applications would make the paper better structured and more balanced. i.e. there is a clear structure: 1) definition of hierrarchy, 2) expressiveness, 3) applications. This way we can also move the welfare maximization preliminaries here and use them in both Algorithmic and PoA sections. It is also a nice merging that here we switch to welfare maximization issues under our hierrarchy.}
\ricomment{looks good}.

A feasible allocation is given by a vector $X=(X_1, \ldots, X_n)$, where $X_i \subseteq M$ denotes the set of items allocated to agent $i$, and $X_i \cap X_j = \emptyset$ for every $i \neq j$. Given a profile of valuations $\vals$, the social welfare (or efficiency) of an allocation $X$ is the sum of the agents' valuations: $SW(X;\vals)=\sum_{i\in [n]}\val_i(X_i)$. Moreover, let $X^*(\vals)$ denote an allocation that maximizes the social welfare with respect to $\vals$; we also call it the optimal allocation for $\vals$ and denote the social welfare of the optimal allocation with $\opt(\vals)$.
When clear in the context we drop the dependence on $\vals$ in our notation and use $X^*$ or $\opt$ to denote an optimal allocation.
%TODO: consider defining the welfare maximization problem. If not, change notations in the algorithm section.

\subsection{Algorithmic Welfare Maximization}
\label{sec:welfare}
\input{algorithmic.tex}

\subsection{Algorithmic Welfare Maximization - Nicole Version}
\label{sec:welfare}
\input{"algorithmic - Nicole.tex"}

\subsection{Welfare Maximization at Equilibrium with Strategic Agents}
\label{sec:poa}
\input{poa.tex}


==> xor-of-or.tex <==
\subsection{XORs and ORs of Single-Minded Valuations}\label{sec:xos-appendix}

\begin{lemma} $\MOPH$-$k$ is closed under OR.\end{lemma}
\begin{proof}

Let $f_1:2^M\to \nonnegR$ and $f_2:2^M \to \nonnegR$ be two $\MOPH$-$k$ set functions. Then we will show that their OR
is also a $\MOPH$-$k$ function. The OR is defined as follows:
\begin{equation}
F(S) = (f_1\vee f_2)(S)=\max_{T\subseteq S}\left( f_1(T)+f_2(S-T)\right)
\end{equation}
Obviously $F$ is monotone whenever $f_1$ and $f_2$ are monotone. Thus it suffices to show that any such $F$ has a positive lower envelope of rank $k$ and it suffices to do show only for the whole ground set $M$. Let
\begin{equation}
T^* = \arg\max_{T\subseteq M}\left( f_1(T)+f_2(M-T)\right)
\end{equation}
Since $f_i$ are $\MOPH$-$k$, each has a positive lower envelope $g_i^T:2^T\to \nonnegR$ of rank $k$ for each set $T$ and we can write:
\begin{equation}\label{eqn:max}
f_i(S) = \max_{T\subseteq M}g_i^T(S\cap T)
\end{equation}
with $f_i(S) = g_i^S(S)$.

Let $G(S)=g_1^{T^*}(S\cap T^*) + g_2^{M-T^*}(S\cap (M-T^*))$. Obviously $G$ is a positive hypergraph function of rank $k$, since it is the addition of two positive hypgraph functions of rank $k$.

We claim that $G$ is a lower envelope of $F$. The no-underestimate property follows easily as
\begin{equation}
F(M) = f_1(T^*)+f_2(M-T^*)= g_1^{T^*}(T^*) + g_2^{M-T^*}(M-T^*)=G(M)
\end{equation}
For a set $S\subseteq M$, we can write:
\begin{equation}
F(S) =\max_{T\subseteq S}\left( f_1(T)+f_2(S-T)\right) \geq f_1(S\cap T^*)+f_2(S\cap (M-T^*))
\end{equation}
Since $S\cap T^*$ is one possible choice in the maximization and $S-S\cap T^*=S\cap (M-T^*)$. By the lower envelope properties of $g_1^{T^*}$ and $g_2^{M-T^*}$, the latter can be lower bounded by:
\begin{equation}
F(S) \geq f_1(S\cap T^*)+f_2(S\cap (M-T^*)) \geq g_1^{T^*}(S\cap T^*)+ g_2^{M-T^*}(S\cap(M-T^*)) =G(S)
\end{equation}
Thus $G$ is a positive lower envelope of $F$ of rank $k$.
\end{proof}


==> xos-k.tex <==
% !TEX root=complements.tex
We next consider the relationship between $\MOPH$-k valuations and the class $\XOS$-k \cite{Sandholm2002}.
This valuation class is represented by combining simple valuations by natural operators.
%For such valuations we need to define the basic elements along with the allowed operators. 
To define $\XOS$-k we require a few basic definitions.
%In the class $\XOS$-k, the basic elements are single-minded-$k$ valuations, and the allowed operators are OR and XOR \cite{sandholm99,LLN}. 
A valuation $v$ is \emph{single-minded-k} if there is a set $S^*$ with $|S^*| \leq k$ and value $v^* \geq 0$ such that $v(T) = v^*$ if $T \supseteq S^*$ and $v(T) = 0$ otherwise. %A single-minded-$k$ valuation is a single-minded valuation where $|S^*| \leq k$. 
We must also define the XOR and OR operations \cite{sandholm99,LLN}.  The formal definition follows, but informally the XOR of two valuations is the maximum among them, and the OR of two valuations is the maximum value obtainable by partitioning a set of elements between them.
%The formal definitions follow.

\begin{defn}
Given two functions $f,g$, the operator XOR is defined as $(f \oplus g)(S) = \max(f(S), g(S))$, and the operator OR is defined as $(f \vee g)(S) = \max_{T \subseteq S}(f(T) + g(S - T))$.
\end{defn}

We are now ready to define the class $\XOS$-k.

%It is easy to see that both operations are commutative and associative. Moreover, the OR operator distributes over XOR: $(a\oplus b)\vee(c\oplus d) = (a\vee c)\oplus (a\vee d) \oplus(b\vee c)\oplus (b\vee d)$ (see Lehman et al. \cite{LLH} for a more extended discussion). Under these observations, 
%One can show that
%any combination of XOR and OR operators on single-minded-$k$
%valuations can always be expressed as a XOR of ORs \cite{LLH}. This motivates the following hierarchy \cite{Sandholm2002} %, which has been used in the literature \cite{Sandholm2002}. 

\begin{defn}[XOR of ORs of Single-Minded-$k$ ($\XOS$-$k$) class] A set function $f:2^M\to \nonnegR$ is in $\XOS$-$k$ if it can be expressed as a XOR of ORs of single-minded-$k$ valuations.
\end{defn}
For the case when $k=1$, both $\MOPH$-$1$ and $\XOS$-$1$ coincide with the class of fractionally subadditive or $\XOS$ valuations. For $k>1$ we show that $\MOPH$-$k$ is strictly more expressive than $\XOS$-$k$. We first show that every $\XOS$-$k$ valuation is also $MOPH$-$k$.

\begin{theorem} 
$\XOS$-$k\subset \MOPH$-$k$.
\end{theorem} 
\begin{proof}
Every single-minded-$k$ valuation is clearly a $PH$-$k$ valuation.
Therefore, in order to prove that $\XOS$-$k$ is contained in $\MOPH$-$k$, it is sufficient to show that the class $\MOPH$-$k$ is closed under XOR and under OR. 
The $\MOPH$-$k$ is closed under XOR follows immediately from its definition, as $\MOPH$-$k$ is defined by a MAX operator. 
The proof that $\MOPH$-$k$ is closed under OR is deferred to Appendix \ref{sec:xos-appendix}.
\end{proof}

On the other hand, we show that there is a large gap in the expressive power of $\MOPH$-$k$ and $\XOS$-$k$.

\begin{prop}
\label{prop:lb-xos-k}
There exists a valuation that belongs to $\MOPH$-$2$ that is not contained in $\XOS$-$k$ for any $k=o(m)$.
\end{prop}
\begin{proof}
\blcomment{I modified this proof, since the prior argument didn't seem to account for the possibility of sets of size less than $k$.  Double-check that this new argument is correct.}
\vscomment{Seems correct to me. Would be great for someone else to also check too.}
Let $v$ be a symmetric valuation such that $v(S) = |S|(|S|-1)/2$ for every $S$. 
The hypergraph representation of $v$ is the function that assigns value $1$ for every set of size $2$, and is therefore in $\MOPH$-$2$.  

Now suppose that $v$ lies in $\XOS$-$k$.
Each single-minded-$k$ valuation in the $\XOS$-$k$ representation of $v$ assigns value at most $|S|(|S|-1)/2$ to its respective set $S$, since otherwise $v(S)$ would be larger than it should be.  Note that this value is at most $(k-1)/2$ per item in $S$, since $|S| \leq k$.
Furthermore, under this representation, the value for $[m]$, the set of all $m$ items, is necessarily expressible as the sum of values of disjoint subsets, each of which has size at most $k$.  %, each of which is assigned a value of at most $k(k-1)/2$ (otherwise, it overestimates the value of a set of size $k$).
Since each disjoint subset can have value at most $(k-1)/2$ per item in the subset, we conclude that $v([m])$ must have a per-item value of at most $(k-1)/2$ as well.  Thus the maximum possible value attainable for $v([m])$ is $m(k-1)/2$.  Since $v([m]) = m(m-1)/2$, it must be that $k=m$.
%Since there can be at most $m/k+1$ such sets, and altogether we need to reach a value of $m(m-1)/2$, it must hold that $(m/k+1) \cdot (k(k-1)/2) \ge m(m-1)/2$, implying that $k=\Omega(m)$, as promised.
\end{proof}


